The HitchHiker's Guide to High-Assurance System Observability Protection with Efficient Permission Switches

Protecting system observability records (logs) from compromised OSs has gained significant traction in recent times, with several note-worthy approaches proposed. Unfortunately, none of the proposed approaches achieve high performance with tiny log protection delays. They also leverage risky environments for protection (\eg many use general-purpose hypervisors or TrustZone, which have large TCB and attack surfaces). HitchHiker is an attempt to rectify this problem. The system is designed to ensure (a) in-memory protection of batched logs within a short and configurable real-time deadline by efficient hardware permission switching, and (b) an end-to-end high-assurance environment built upon hardware protection primitives with debloating strategies for secure log protection, persistence, and management. Security evaluations and validations show that HitchHiker reduces log protection delay by 93.3--99.3% compared to the state-of-the-art, while reducing TCB by 9.4--26.9X. Performance evaluations show HitchHiker incurs a geometric mean of less than 6% overhead on diverse real-world programs, improving on the state-of-the-art approach by 61.9--77.5%.

==> tex/daemon_realtime.tex <==
\section{\codename Daemon: Guaranteed Task Execution}
\label{sec:daemon_realtime}

As HD is dedicated to log management, its performance is essential to ensure the whole system's efficiency.
The protection scheme is triggered per time $T_p$ to secure a current buffer.
Therefore, HD is responsible for consuming the protected buffer and refilling the buffer pool timely, preventing system block due to buffer exhaustion.

\subsection{Multithread Task Execution}
During process initialization (\cref{subsubsec:deterministic_process_initialization}), HD entrusts two threads (as shown in \cref{fig:workflow}) for log management:
\textbf{Receiver thread} is responsible for consuming logs from the protected buffer to its \textit{internal thread shared buffer} (\circlewhite{1}--\circlewhite{2}).
Once a log buffer is consumed, it requests the SM (\hwno{6}) to return it to the kernel buffer pool by allowing the buffer's access permission from the \Aa{GPT}{NS} (\circlered{1}--\circlered{\Aa{2}{b}}).
\textbf{Manager thread} is to manage logs.
It requests the secure monitor to persist logs into protected storage (via the abstraction \hwno{9}).
Also, the remote administrator can query logs via a network interface.
Recall that HD relies on the native OS for resource (e.g., network) management.
Thus, HD depends on OS services (e.g., \texttt{send}) for its tasks (\cref{subsubec:restricted_os_services}).

\codename segregates the log buffer consumption and log management into above two threads.
By this way, it ensures the heavy managment jobs (i.e., I/O and network) is dispatched to the manager thread.
Thus, the log buffer pool is renewed in time by the receiver thread to avoid system block due to the its exhaustion.
Moreover, two threads use \texttt{atomic} operations to process their shared buffer (during \circlewhite{2}--\circlewhite{3}).

\noindent\textbf{Thread management.}
Still, HD depends on OS service (i.e., \texttt{clone} and \texttt{futex}) for thread creation and synchronization (\cref{subsubec:restricted_os_services}).
Specifically, during thread creation, the SM interposes \texttt{clone} with the flag \texttt{CLONE\_VM}, to record the child thread's TID and configure its address space and stack.
Also, the HD threads' stacks are deterministically mapped to the preserved region during initialization.
After all threads are created, the SM verifies HD's page table (\hwno{1}) and ensures that all pages are mapped to the expected locations.

% Where to say that?
% All the primitive abstraction requests from the HD should be authenticated by the SM (as denoted in~\cref{tab:hw_abstraction}).
% This can be achieved by generating a secret token inside the HD's physical memory during secure boot~\cite{cerdeira2022rezone}.
% The trust gateway then verifies the token passed as a parameter.
% By doing so, the SM ensures the HD's integrity (e.g., a malicious OS can not impersonate the HD to switch a log buffer's access permission via \hwno{6} or issue malicious I/O job via \hwno{9}).

\subsection{Guaranteed Task Execution and Scheduling}
The performance of HD is critical to \codename's full system performance.
HD's log consumption throughput is the bottleneck of the whole system, as the system will be blocked if the buffer pool is exhausted.
Thus, HD's execution should be guaranteed by the SM.

\noindent\textbf{Prioritized execution.}
\codename prioritizes HD's threads execution by assigning \texttt{MAX\_RT\_PRIO} to HD threads' scheduling policy.
Moreover, the CPU affinity of HD's threads is configured to a dedicated core upon process initialization (\cref{subsubsec:deterministic_process_initialization}) to avoid interference from other tasks.

\noindent\textbf{Non-preemptible execution.}
When HD is executing, the core's inter-processor interrupts (IPIs) are disabled.
Meanwhile, all hardware interrupts, except the protection scheme timer and the protected storage's interrupts, are disabled.

\noindent\textbf{Task scheduling.}
Once a HD-requested OS service is finished (\cref{subsubec:restricted_os_services}) or the scheduler decides to wake up HD, SM takes charge of the CPU context switch (\hwno{4}) by intercepting \texttt{kernel\_exit} (\circleblack{C}--\circleblack{A}).
Then, SM activates \Aa{GPT}{HD} by configuring \texttt{GPTBR\_EL3} (\circlered{1}) to access \Aa{M}{HD} and switches CPU contexts to HD.
During HD's execution, when there is no log to consume or manage, its threads sleep, allowing the CPU to be scheduled by other tasks.


==> tex/daemon_tcb.tex <==
\section{\codename Daemon: Dedicated Runtime Secure Environment with Small TCB}
\label{sec:daemon_tcb}

% \adil{consider a special name for your environment.}\chuqi{HD? HitchHiker Daemon as the title?}

After in-memory observability protection, a secure environment: \codename daemon (HD) is required to manage logs~--~batching them for persistence and support remote administrator access. 
As stated in~\cref{subsec:design_choices}, HD is a dedicated environment to log management with limited but necessary execution interfaces. 
Instead of deploying a trusted kernel, \codename relies on its native OS for task scheduling and services to minimize its TCB and ensure the its near-native performance.
% This is a common practice~\cite{hof2022blackbox,zhang2023shelter} in recent works.
SM enforces HD's isolation by configuring essential primitive abstractions and managing its lifecycles.

% \chuqi{Mention about capability?}
\subsection{Deterministic Process Initialization}
\label{subsec:deterministic_process_initialization}
The binary of HD, as well as its exception vector table, are statically built without any dynamic links.
Hence, its binary image (ELF) is verifiable by the SM (e.g., via hash) during loading.
Before the secure boot, HD's memory is statically preserved to a fixed physical region (\Aa{M}{HD} in~\cref{fig:workflow}) by editing the device tree.
M{\scriptsize{HD}} is not accessible by the NS due to the GPT{\scriptsize{NS}} permissions.
During process initialization, the SM interposes its process virtual memory setup in kernel (e.g., \texttt{elf\_map}) to map the binary image (e.g., its stack, code, and data sections) to the preserved \Aa{M}{HD}.
By doing so, the SM ensures HD's virtual memory space is always \textit{prepaging} to the determined space instead of \textit{demand paging (lazy allocation)}.
Therefore, its initial page table can be shadowed by the SM (\hwno{1}) for further verification.
Similarly, its exception vectors are loaded and mapped to a fixed region during initialization (\hwno{2}).

\subsection{Restricted OS Services}
\label{subec:restricted_os_services}
HD may require the OS services, like syscalls for network access and interrupt handling, to finish jobs.
Unlike existing works~\cite{hof2022blackbox,zhang2023shelter}, the HD is dedicated to log management.
Its OS service interface is restricted by the SM to minimize the attack surface like memory-based Iago attacks~\cite{stephen2013iago}.
Before OS invocation, HD always invokes the SM (\hwno{3}) by forwarding its exceptions to the trusted gateway (\circlewhite{A}--\circleblack{A}) for inspections:


\noindent\textbf{Immutable memory layout.}
HD's memory layout is immutable \textit{after} its initialization (\cref{subsubsec:deterministic_process_initialization}).
During execution, memory allocation or remapping (e.g., \texttt{mmap} from its exceptions) is not allowed by SM.
Therefore, after process initialization, HD's page table and exception vectors are immutable.
This prepaging strategy of HD avoids page faults and page remapping during execution.
Further, the trusted gateway ensures that by inspecting the \texttt{ESR\_EL1} register and exception offset.
By this way, \codename ensures the integrity of HD's memory layout that the OS can not remap its pages.

\noindent\textbf{Limited syscall support.}
After HD's initialization, SM only supports limited syscalls for HD to perform necessary services like thread and network management.
That is, HD is not allowed to request arbitrary syscalls (e.g., \texttt{mmap} for memory allocation or \texttt{fstat} for file checks).
To support allowed syscalls, the SM re-prepares pointer parameters of syscalls (e.g., the \texttt{buf} of \texttt{send}) to a shared memory for OS.
Before entering OS, the SM activates \Aa{GPT}{NS} by configuring \texttt{GPTBR\_EL3} (\circlered{1}) to enforce memory isolation.
After those security checks, the service is further forwarded to the OS (\circleblack{B}--\circleblack{C}).


==> tex/design-old-1.tex <==
\section{\codename Design}
\label{sec:design}
%

%
This section describes the main challenges towards \codename's design, and the following sections describe how we address them.
% 

% \PP{C1: Enforcing protected domains with hardware primitives.}
% %
% The secure environment is kept isolated from the untrusted system.
% %
% Without leveraging general-purpose components like hypervisor or the TrustZone, it is challenging to abstract the domain isolation (memory and device) enforcement from hardware features.

\PP{C1: Reducing software porting and deployment efforts.}
% 
Given strict requirements to ensure high assurance, it is challenging to design an infrastructure where these strategies are satisfied without significant deployment effort (\eg completely rebuilt storage drivers for persistence or natively support the daemon).

% \chuqi{check}

% An observability protection system requires an overhaul of the conventional OS-maintained software infrastructure.
% %
% It is challenging to involve minimal extensions of the conventional software stack and reduce the deployment efforts (\cref{subsec:design_security_monitor}).\adil{your system is making lots of changes to the conventional stack. This will go against you.}
\PP{C2: Enforcing short multi-layer log protection deadlines.}
% 
Unlike prior work that only deals with OS logs, protecting logs from different layers, including applications and network logs, and under the (at least unprivileged) access of an adversary, makes it challenging to enforce uniform and very short deadlines.

\PP{C3: Delegating log management to untrusted OS securely.}
% 
Any task naively delegated to the OS becomes untrustworthy after its compromise. 
% 
Since it is agnostic to administrators when the OS is compromised, the OS can provide completely wrong responses after compromise even without tampering with logs.

% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Secure Environment Setup and Bootstrap}
% \subsection{Secure Environment Intialization}
% \subsection{Secure High-Assurance Environment Setup}
% \subsection{High Assurance Environment Software Stack}
\subsection{High Assurance Secure Software Stack}
\label{subsec:design_security_monitor}
%

\codename maintains its secure software stack with (a) the security monitor to enforce memory and device isolation, (b) a protected device driver to guarantee log persistence, and (c) an enclave log daemon process for log management.
%

This section first explains how \codename security monitor enforces its isolated environment.
%
Then, it explains how software components are created and deployed into the system.

% We explain their setup, initialization, and execution in the remaining paragraphs.

% \codename minimally extends the conventional observability stack with log protection components (\cref{subsec:overview_secure_environment}).
% %
% In this section, we describe how their initialization and overall workflow.\AD{Fix grammar. Say something more useful here. Do you really explain "minimally extends" in this section?}
% It is inspired by {\em privileg-monitor-based} solutions~\cite{varun2023omnilog,shepherd2017emlog}.
% \AD{Rewrite para}

% %
% First, it deploys a security monitor {\bf \codename\ Monitor (\sm)} at EL3 (management mode).
% %
% Second, a dedicated log storage device is used by a {\bf protected and debloated driver} for log persistence.
% %
% With driver debloating techniques~\cite{guo2022driverlet}, \codename automatically creates and installs a debloated storage driver.
% %
% Last, a {\bf \codename\ Daemon (\hd)} is devised as a protected userspace daemon (compatible with the OS) for log management.

% secure environment is inspired by {\em privileged-monitor-based} solutions~\cite{varun2023omnilog,shepherd2017emlog}---containing a privileged security monitor ({\em \codename Monitor, \sm}), a log managing daemon {(\codename Daemon, \hd}), and a {secondary protected log storage device}.
% % 
% However, instead of designing a new hardware layer for its monitor, \codename employs the privileged EL3 (SMM), which is kept small.
% % 
% Moreover, instead of redesigning a storage driver, \codename leverages a debloated driver inside the \sm.
% % 


% % 
% alongside a {\em native but secured user-space} daemon for \hd (\cite{varun2023omnilog,shepherd2017emlog} use commodity trusted kernels).
% % 
% Unlike VMMs and TZ, EL3 is purposefully kept very small (\cref{sec:arm_background}), and provides a narrow interface (through \textcode{SMC}s) to the OS. 
% % 

%%
% \PP{Offline debloated driver template synthesis.}
% %
% \codename provides an offline tool to synthesize a debloated storage template prior 
% to system bootstrap, which is later instantiated into \sm during its initialization. 
% %
% This is done by using record-and-replay mechanisms~\cite{wang2022rttee,guo2022driverlet} for storage drives (\eg SATA, USB, etc), as a one-time effort.

% % 
% Our record-and-replay tool considers a storage device as a finite state machine (FSM).
% %
% Hence, the operations of a driver 
% are distilled into a sequence of {\em driver-device} interactions, each of which is a FSM transition.
% % 
% These interactions remain consistent irrespective of the I/O task payload variations~\cite{guo2022driverlet} to be recorded into a {\em template}.
% %
% In particular, during the recording phase, we issue sample I/O jobs to log storage and templatize the following interactions (detailed in \cref{sec:impl}):
% % 
% (1) the sequences and content of Memory-mapped I/O (MMIO) write operations to the log storage, 
% (2) the allocation of direct-memory-access (DMA) buffers for the log storage, and 
% (3) interrupt request (IRQ) numbers invoked by the log storage, along with the completion status.
% %
% The template is then installed into \sm's binary.
% %
% Note that the recording phase is a one-time effort from an administrator's perspective.

% \PP{System memory layout reservation}
% \PP{System memory domains creation}
% \PP{Memory protection domain enforcement}
% \PP{EL3 monitor with GPT/SMMU protection}
% \PP{SMM-based monitor with GPT/SMMU protection}
% \chuqi{top-down in below section}

% \vspace{-0.2cm}
\PP{Security monitor with enforced protection domains}
\label{subsubsec:security_monitor}
%
The security monitor (\sm) dynamically configures the {\em hardware memory permission primitives}, as mentioned in \cref{subsec:overview_inmemory_observability_protection}, to protect both \codename's secure environment components and runtime logs.
%
% \footnote{TZASC's static setup and limited region count~\cite{li2021twinvisor} lacks flexibility.
% %
% Therefore, we design and implement \codename using both S2PT and GPT. 
% %
% See discussion in~\cref{sec:discussion} to understand their implications and alternative features on other platforms.}.
%
% It executes within the SMM software, like a runtime component of ARM Trusted Firmware or UEFI, which is securely loaded during trusted boot~(detailed in \cref{sec:impl}).
It is securely loaded during the trusted boot~(detailed in \cref{sec:impl}).

% 
During initialization, \sm creates memory protection domains: 
% 
one for its own memory regions and \hd's regions (trusted), 
% 
and the other for regions for untrusted components---the host OS and all its applications (untrusted).
% 
\sm prevents malicious CPU access to trusted domains by leveraging memory permission primitives.
% 
% \sm creates and maintains two GPTs within \domsm: one where untrusted component regions (\domu) are marked accessible and another where \hd's regions (\domhd) are marked accessible.
%
To be specific, \sm maintains {\em two memory-permission-views}: one where {\em only} untrusted component regions are marked accessible, and the other where \hd's regions are marked accessible.
%
% \sm is marked as {\em read-execute-only} in both views.
%
This is achieved by maintaining separated memory permission configurations for different domains.
%
Specifically, \sm uses two separate S2PTs or GPTs for the untrusted and the trusted domains, and activates the corresponding configuration during {\em runtime domain transitions}.

% \domsm is also marked accessible in both GPTs, allowing domains to call \sm for a service~(\eg log protection).
% 
% This is secure since, within both GPTs, \sm regions are marked as {\em root} (\cref{sec:arm_background}), which allows their access in the EL3 CPU execution mode {\em only}.
% 
% This allows \sm to modulate memory views, ensuring that CPUs can only access their dedicated memory in specific execution modes.
%

\sm prevents malicious device (DMA) access to trusted domains using the System Memory Management Unit (SMMU)~\cite{varun2023omnilog,sridhara2023acai}, which limits the addressable physical memory of a device.
% 
SMMU interfaces (stream tables and request-response buffers), are protected within \sm (by aforementioned permission restrictions).
% 


% \sm also interposes all domain transitions to ensure correctness.
% % 



% \sm divides the system into 4 memory regions (the left table in~\cref{fig:workflow}).
% %
% \begin{enumerate}[leftmargin=*,label=\textbullet]
%     %
%     % An untrusted OS can only access this region at runtime.

%     \item
%     {\bf{\Aa{M}{\sm}\xspace}} is where \sm resides,  alongside its permission switch primitives (\ie GPT configurations) and the aforementioned debloated driver.
%     % 
    
%     % , and other platform-generic security services~\cite{atf}.
    
%     \item
%     {\bf{\Aa{M}{\hd}\xspace}} is the reserved physical address space for \hd, including its binary sections and execution stacks.
    
%     \item{\bf{\textsc{Mbufpool}\xspace}} is an in-kernel buffer pool designated for log capture and runtime permission switch.

%     \item
%     {\bf{\textsc{Mut}\xspace}} is the region for the untrusted system domains (\ie host OS, all its applications, and normal driver interfaces).

% \end{enumerate}

% \adil{4 memory regions and only 2 GPTs is confusing.}
% \chuqi{Mut is Dut, Mhkd and Mhkm are Dt, Mbufpool are dynamically between Dut and Dt?}

% Once setting up the system layout, \sm configures memory protection mechanisms to isolate the secure environment from the OS (explained in the following).

% \PP{Memory-view partition and isolation.}
% \PP{Protected memory region initialization.}
% \PP{Reserved memory region protection}
% % 
% \sm configures GPT and System Memory Management Unit (SMMU) to isolate the secure environment memory regions from untrusted domains CPU and device DMA access, respectively.

%
% To isolate untrusted OS' CPU memory access to the secure environment, \sm creates and maintains two GPTs~\cite{sridhara2023acai,zhang2023shelter,hof2022blackbox}: one for the untrusted system ({\sc GPTut}) and the other for the trusted components ({\sc GPTtr}).
% %
% This allows \sm to modulate memory views, ensuring that CPUs can only access their dedicated memory in specific execution modes.
% %

% As noted above, both \domu and \domhd can call \sm for a service. 
% % 
% This is achieved using an \textcode{SMC}~(\cref{sec:arm_background}).
% % 
% A special \textcode{SMC} is also used to transition between domains (\eg when the OS schedules \hd).
% % 
% In such calls, \sm swaps the GPT pointers in the \textcode{GPTBR\_EL3} register and returns to the target domain.
% % 
% Please refer to \cref{subsec:design_daemon} for additional details.
% % 

% When a CPU operates in untrusted domains (OS and applications), {\sc GPTut} {\em always} restricts its permissions to the secure environment, confining it to the {\sc Mut} (see memory views in \cref{fig:workflow}).
% %
% \sm, during runtime, performs security checks and changes the activated GPT for CPU context switches between domains (\cref{subsec:design_daemon}).
% %
% \adil{Chuqi, can you explain this better?}

% Apart from confining CPUs' memory permissions by GPT checks during MMU walks, \sm also addresses DMA access configuration
%  for devices to prevent DMA attacks.
% %
% To do so, \sm configures SMMU to limit device memory permissions~\cite{varun2023omnilog,sridhara2023acai}.
% %
% Moreover, the SMMU configuration interfaces (\eg control registers and stream tables) are then protected in \sm~\cite{sridhara2023acai} 
% by {\sc GPTut} (\ie the untrusted domains can not tamper with SMMU configuration).
%
% This concept aligns with common practices~\cite{hofmann2013inktag,hof2022blackbox,zhang2023shelter,sridhara2023acai} that leverage permission primitives for physical memory space access control

% \adil{why do we need this sentence? Avoid talking about existing work in design.}\chuqi{removed}
%
% By doing so, our system is an extension of the CCA Realm world, which is orthogonal to the original purpose and doesn't require any modification of its own codebase (discussed in APPEN.X)~\cite{sridhara2023acai,zhang2023shelter}.
% \adil{Is it really an extension? It's not clear how/why at this point. Clarify.}\chuqi{removed}
\vspace{-0.1cm}\subsubsection{\textbf{Debloated driver synthesis and initialization.}}
\label{subsubsec:debloated_driver}
%
\codename provides an offline tool to synthesize a debloated driver prior 
to system bootstrap, which is later instantiated into \sm during initialization. 
%
This is by record-and-replay mechanisms~\cite{wang2022rttee,guo2022driverlet} for storage drives (\eg SATA, USB, etc), as a one-time effort.

% 
Considering a storage device as a finite state machine, driver operations are distilled into a sequence of {\em driver-device} interactions, each of which is a state transition.
% 
These interactions remain consistent irrespective of variations in I/O workloads~\cite{guo2022driverlet}.
% to be recorded into a {\em template}.
%
During recording, sample I/O jobs are issued to log storage to templatize the following interactions (detailed in \cref{sec:impl}):
% 
% (1) the sequences and content of Memory-mapped I/O (MMIO) write operations to the log storage, 
% (2) the allocation of direct-memory-access (DMA) buffers for the log storage, and 
% (3) interrupt request (IRQ) numbers invoked by the log storage, along with the completion status.
(1) memory-mapped I/O (MMIO) write operations to the log storage,
(2) DMA buffers allocated for the log storage,
and 
(3) interrupt request (IRQ) by the log storage.
%
The template is then installed into \sm.
%
% Note that the recording phase is a one-time effort from an administrator's perspective.

% While there are other choices, like porting and isolating a driver into \sm via memory-safe language, we choose the driver record-and-replay due to (a) easy-of-verification given such a debloated driver, and (b) easy-to-deploy as it can be automatically recorded (explained in \cref{subsec:design_offline}).
% %
% Nonetheless, the other approaches can be applied as well in the future.


% \PP{Log storage disk initialization.}
%
\sm sets up the debloated driver from the template during initialization to enable communication with the log storage disk.
%
Specifically, the driver's MMIO regions (which are fixed physical addresses) and allocated DMA buffers are only mapped to monitor's memory region.
% 
% Recall that this region is protected by permission and SMMU. 
%
% Hence, the untrusted OS cannot manipulate protected driver interfaces.
Thus, the untrusted OS cannot manipulate the driver interface.
% 
To ensure interrupts from the log storage disk are routed to the protected driver only, \sm updates the IRQ table in the EL3 interrupt management framework~\cite{irqroute}.
% 
At runtime, \sm replays the template with dynamic parameters (\eg MMIO control sequences with DMA payloads) to read or write disk sectors.
%

\vspace{-0.3cm}
\subsubsection{\textbf{Protected userspace log daemon execution}}
\label{subsubsec:daemon_execution}
% 
\codename enables loading a user program (\hd) into a protected userspace process (or enclave) for log management.
% 
The process maintains OS compatibility, allowing developers or administrators to build log management functionality easily.
% 
The remaining paragraphs in this heading describe how \hd is collaboratively loaded and secured during execution, while \cref{subsec:design_daemon} explains how remote log management tasks are authenticated and secured using \hd.
% 
% \sout{Note that supporting our protected userspace process requires very minor changes to the kernel, the majority of which are isolated within a loadable module in our implementation~(\cref{sec:impl}).}
% 

\PP{Collaborative loading.}
%
\hd's collaborative loading is inspired by SGX ~\cite{mckeen2013sgx} and recent research~\cite{hof2022blackbox,hofmann2013inktag,zhang2023shelter}.
% 
% \sout{Prior to deployment (during machine provisioning), \hd is compiled with all required libraries in a statically-linked manner.
% % 
% This avoids insecure code-sharing with OS-controlled libraries.}
% 
% At machine provisioning, it is installed within the protected disk by the administrator.
%
% During system boot, the monitor reads its binary and provides it to the OS, which allocates a process context and loads the binary within a reserved region.
%
% \sm verifies the integrity of the loaded binary by comparing its contents with a pre-installed SHA-256 cryptographic integrity hash.
At machine provisioning, its binary SHA-256 integrity hash is pre-installed onto protected storage.
%
During system boot, the OS allocates its process context, loads the binary within a reserved region, and requests \sm to attest to its initial integrity (\ie via the pre-installed hash).
%  
To prevent {\em time-of-check-to-time-of-use} attacks, the monitor protects the process region (by domain enforcement in \cref{subsubsec:security_monitor}) before verification.
% 
Once the binary is attested, the monitor then copies the page tables of the process into its own memory region.
% 

%
After attestation, \hd's pages are {\em pinned} to memory (\ie no swapping). 
%
As \hd's page table is maintained inside the monitor's memory, the OS cannot make any changes to verified mappings, thereby preventing page remapping attacks~\cite{hofmann2013inktag}.
% 
Pinning is acceptable since \hd would typically only require a small amount of memory~(less than 8MB in our implementation).
%

\PP{Execution and scheduling.}
\hd is initialized with two threads: a {\em consumer} and a {\em manager}.
% 
The former is used to consume protected logs, while the latter is used to issue log persistence operations (\cref{subsec:design_realtime_deadline}) and securely respond to remote tasks (\cref{subsec:design_daemon}).
% 
Like any process, the scheduling of \hd is controlled by the OS.
% 
However, the OS cannot directly transition into \hd's context, which is protected by the monitor.
% 
Hence, whenever the OS wants to schedule one of these threads, it calls the monitor using a Secure Monitor Call (SMC~\cite{smccc}).
% 
In such calls, \sm swaps the memory-view to \hd and returns to the target thread, with the protected page table.
% 
% At this time, \sm also sets the thread's secure page table (which is copied to \sm during loading).
% 

Once scheduled, \hd cannot exit directly to the OS for system calls or interrupts due to domain enforcement (\cref{subsubsec:security_monitor}).
% 
Hence, to securely and transparently support system calls and interrupts during \hd's execution,
% 
\sm installs a custom exception vector table whenever an \hd thread is scheduled, in which all exceptions are interposed by a trampoline SMC (\cref{fig:workflow}, \circlewhite{A}--\circleblack{A}).
%
On that transition, the monitor saves \hd's context before exiting to the OS (\circleblack{B}).
% 
Whenever the OS calls the monitor to reschedule the \hd, the context is restored (\circlewhite{B}).
%
Like typical enclaves, it is the program's responsibility to ensure that system call results are sanitized to prevent IAGO attacks~\cite{stephen2013iago} (\eg OS returns a malicious pointer).
% 
We explain how network system calls are sanitized in~\cref{subsec:design_daemon}.
% 
In the future, if other system calls are needed by the program, a small TCB-conscious Library-OS~\cite{tsai2017graphene,shinde2017panoply} can be integrated with \hd.
% 

% \sm correctly sets its page and vector tables by \textcode{TTBR0\_EL1} and \textcode{VBAR\_EL1}, respectively.
% Please refer to XX to understand how \hd's threads communicate with \sm and the OS.
% % 

% 
% \sm retrieves the \hd binary from the protected disk and sends it to the OS for installation.
% % 
% \sm can simply install the binary itself, but this would unnecessarily bloat and complex \sm's TCB.
% % 
% Instead, OS loads the process and sets up its virtual space mapping to an OS-allocated region during loading, \sm verifies the correct layout of its binary.
% % 
% This is similar to how remote users attest that an SGX enclave~\cite{mckeen2013sgx} is correctly installed by the OS.
% %
% % 
% To prevent time-of-check-to-time-of-use (TOCTOU) attacks, the OS-allocated region is protected in \domhd once the page is set up (using \sm's domain enforcement) before verification.
% % 
% If verification fails, the OS is considered malicious, and logging is halted with a warning log message.
% %
% OS also pre-allocates and sets up the execution stacks for \hd thread initialization, and calls \sm to verify and protect their stacks in \domhd.



% %
% Once installed, \sm maintains the page tables of \hd.
% %
% The initial page table mappings are provided by the OS, but are also verified using the process mentioned in the last paragraph.
% % 
% After verification, \hd's pages are {\em pinned} in memory. 
% %
% As its page table is maintained inside \domsm, the OS cannot make any changes to the verified mappings to perform page remapping attacks~\cite{hofmann2013inktag}.
% % 
% This is acceptable since \hd would typically only require a small amount of reserved memory~(less than 16MB in our implementation).
% %



% 
% The OS allocates a region of memory for \hd.
% % 
% \sm leverages its memory domain enforcement mechanisms (previous heading) to protect this region in \domhd.
% % 
% \sm then retrieves the \hd binary from the protected disk, and securely loads the binary pages into the protected region.
% 

% \sm interposes \hd's binary load (through a specialized kernel module) during initialization, to attest to its correctness and protect it.
% % 
% During the virtual address space setup, \sm creates and maintains the page table of \hd, mapping its address space to the reserved region \Aa{M}{\hd}.
% %
% To prevent time-of-check-to-time-of-use (TOCTOU) attacks, each page mapping is protected and fixed before verification.
% %
% Then, \sm verifies each page using an SHA-256 cryptographic hash~(like SGX enclaves~\cite{mckeen2013sgx}) and compares the final measured hash against a pre-determined value.
% % 
% If the comparison is false, the OS is considered malicious, and logging is halted with a warning log message.
% % 
% %
% After verification, \hd's pages are {\em pinned} in memory. 
% %
% As its page table is maintained inside \domsm, the OS cannot make any changes to the verified mappings to perform page remapping attacks~\cite{hofmann2013inktag}.
% % 
% This prepaging is acceptable since \hd does not require a significant amount of memory or dynamic memory updates.

% \PP{Log buffer pool and timer specification.}
% %
% A dynamic buffer pool is maintained for the capturer, wherein the permissions of each buffer are switched based on a timer-defined real-time deadline.
% %
% %
% \codename promptly pops the {\em current log buffer} from the pool for protection (\cref{subsec:design_realtime_deadline}), and concurrently consumes the buffer in the background \hd, subsequently placing it back to the pool (\cref{subsec:design_daemon}).
% %
% \codename's hardware timer is activated once the observability capturer is enabled.
% %
% Since the OS is initially benign after the secure boot, the timer is correctly deployed before the OS compromise ($t_c$).

% \chuqi{To be shorten: record-and-replay and storage initialization filled too much space}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/workflow_short.pdf}
    % \vspace*{-0.7cm}
    \caption{
    \codename workflow and components.
    %
    \codename\ {\em Monitor} (\boxsm\ \sm) and {\em Daemon} (\boxhd\ \hd) are trusted.
    } 
    \label{fig:workflow}
    \vspace{-0.4cm}
\end{figure}

\subsection{Deadline-Enforced Unified Log Protection}
\label{subsec:design_realtime_deadline}


% A reliable, periodic hardware timer for log protection allows an administrator to configure a real-time protection delay of $T_p + \epsilon$, where $T_p$ is the timer interrupt frequency and $\epsilon$ is the latency incurred while protecting logs in memory.
%
\codename\ {\em enforces} the unified short log protection deadline by employing a reliable, periodic hardware timer.
%
The administrator configures a real-time protection delay of $T_p + \epsilon$, where $T_p$ is the timer interrupt frequency and $\epsilon$ is the latency incurred while protecting logs in memory.
% 
Hardware timers today have a high resolution~\cite{wang2022rttee}; hence, $T_p$ can be tiny (\eg \textus{100}--\textms{1}).

% 
This section first explains how different logs are collected in a unified location to standardize the timer protection window.
%
Then, it explains how the timer is controlled to ensure the collected logs are protected in memory within a set deadline.
%
Finally, it concludes with a description of how protected logs are securely persisted in the background to guarantee eventual availability.
%

% Without the log persistence guarantee, the in-memory protection would be futile as logs can be dropped after the system powers off.
%
% \adil{Please shorten intro into 3-4 lines (high-level).}
% \chuqi{check}

% \PP{Log buffer pool and timer specification.}
%

% 
% %

% \adil{Merge this and the next heading into one heading that describes (a) how the kernel keeps a log buffer pool and (b) how all logs are collected within the buffers. You should shortly mention eBPF here, since its part of your figure, and its not obvious how you collect logs in a unified manner otherwise. Move the timer aspecs into the "hardware timer-..." heading.}


% \PP{Unified log capture in singular buffers.}
% \PP{Log buffer pool-based unified capture.}
\PP{Unified log collection in kernel buffer pools}
%
Capturing logs at different locations (\eg network drivers, applications) in an ad-hoc manner and protecting them can increase protection delay.
% 
\codename avoids this by unified capturing logs within the kernel before protection~(\circleblack{1}--\circleblack{2} in~\cref{fig:workflow}).
% 
It requires two aspects for unification: (a) a central region (buffer) to hold logs and (b) a mechanism to generate the captured events as logs to that region.
% 

% 
To create a central region, \codename allocates a {\em pool of per-core} buffers within the kernel observability generator's memory.
% 
For each kernel thread, logs are always written to the {\em current} per-core buffer within the pool, thereby avoiding cross-core contention as multiple kernel threads can write logs simultaneously.
%

%
A per-core pool of (at least two) buffers is required, because \codename dynamically switches the {\em current} buffer's domain for protection (as explained in the next heading).
%
Hence, there should always be an available buffer to serve as the {\em current}.
% 
The size of the buffers is administrator-controlled.
% 
If the buffer becomes full, very rare in honest scenarios based on proper configuration in our evaluation~(\cref{sec:performance_evaluation}) and prior work~\cite{varun2023omnilog}, the generator waits for a buffer to be consumed and returned.
% 
This prevents attackers from overwriting their attack trace even if they generate many spurious logs from userspace~\cite{riccardo2020kennylogging} before full system compromise.
% 

% For generating logs, our implementation leverages eBPF~\cite{ebpf,tracee}~(more details in~\cref{sec:impl}).
% % 
% Note that this can be easily ported to other tools like KLogger~\cite{yoav2007klogger} and can support extra log sources through diverse probes (discussed in~\chuqi{X}).
% % 

\codename collects the logs (\circleblack{1}) by extended Berkeley Packet Filter~(eBPF)~\cite{ebpf}, which is widely-used in prior work~\cite{agman2021bpfroid, minna2023sok}.
% 
A challenge in capturing {\em application logs} is locating and automatically intercepting the routines where logs are generated.
% 
\codename addresses this by using contextual tracking of file system calls.
% 
In particular, applications leverage the OS file system to write logs. 
% 
Thus, the generator records {\em write} syscalls and extracts file paths in kernel structures (\eg \textcode{dentry} in \textcode{vfsmount}) to match them with administrator-defined log file paths (\eg \textcode{/var/log})~\cite{tracee}. 
% 
For log file writes, \codename extracts the log string using an eBPF helper \textcode{bpf\_probe\_read\_user}.
% 
% In contrast to application logs, \codename generates and collects logs from network and system calls directly ~(\circleblack{2}).
% , \codename leverages the extended Berkeley Packet Filter~(eBPF)~\cite{ebpf}, like prior work~\cite{agman2021bpfroid, minna2023sok}. 
%
For logs from network and system calls, \codename injects BPF programs into kernel tracepoints to attach all 436 system calls and socket-related events.
%
\codename follows Linux Auditd's format~\cite{auditd} to generate system call log entries, which include parameters, return values, and other fields (\eg process identifiers and timestamps).
% 
For network traffic logging, \codename logs IP, ports, and other packet data from the kernel socket structure of network traffic.
% 



% A buffer pool is maintained for the capturer, wherein the permissions of each buffer are switched between {\domu and \domhd} dynamically.
% %
% The capturer records multi-layer observability logs from the kernel.
% %
% To unify their protection window, \codename captures all logs within the same kernel buffer before protection.
% 

% \chuqi{leave to implementations}
% % 



% Our implementation leverages eBPF~\cite{ebpf,tracee} for observability capturer~(more details in~\cref{sec:impl}).
% % 
% Note that this can be easily ported to other tools like KLogger~\cite{yoav2007klogger} and can support extra log sources through diverse probes (discussed in~\chuqi{X}).
% \adil{(e.g., write, fwrite, fput)}\chuqi{honestly only write are typically used in app. logs. fwrite and fput are not syscalls but libc funcs.} 
% \adil{Minor: How do you correlate?}\chuqi{fixed. it's predefined by administrators}

% \adil{can you have a heading here talking about how you handle the (16?) buffers? You also need to mention that you pause execution if buffers become full.}\chuqi{fixed}

% \adil{Unprolongable is not a word. Heading is not about the guarantees, its about how you enforce them. The section heading already says "deadline".}

% Given the deadline of $T_p + \epsilon$, the $\epsilon$ is always kept small and regular for buffer protection (context switches and GPT configurations shown in~\cref{tab:prot_primitives}), 
% %
% In other words, attackers shall not prolong this deadline during system exploitation.

% \PP{Prompt timer response with no drop protection.}
% \PP{Hardware timer-initiated buffer protection.}
\PP{Controlled hardware timer-based buffer protection.}
%
The OS deploys a hardware timer based on configured frequency $T_p$ to direct a kernel thread to initiate log protection.
% 
As the OS is initially benign after the secure boot, the timer is correctly deployed before the OS compromise.
% 
\codename~{\em controls} the delay after the timer expires to ensure that protection is achieved within a regulated small period ($\epsilon$).
% 
This ensures that each log's protection deadline is $T_p + \epsilon$.
% 
All these aspects are explained in the next paragraphs.
%

%
Once logs are captured, \codename writes them to the {\em current} buffer~(\cref{fig:workflow}, \circleblack{\Aa{3}{a}}). 
%
When a timer deadline is reached, a kernel thread calls \sm (\circleblack{\Aa{3}{b}}--\circleblack{A}) to temporarily switch the current buffer's domain from the untrusted to trusted (\circlered{1}--\circlered{\Aa{2}{a}}).
%
After protection is complete, a new buffer is fetched from the pool to become the new {\em current} buffer (\circleblack{B}--\circleblack{\Aa{3}{c}}).
% 
The previous (now protected) buffer will be re-inserted into the pool after consumption~(next heading).

% \adil{explain in next heading?}
% After the protected buffer is consumed, its domain switches back to \domu to re-add to the pool~(explained in the next heading).
% %
% If all buffers are exhausted or full, the CPU context associated with the log event is paused to prevent log drop~\cite{ahmad2022hardlog}, until a protected buffer's permission is returned by \hd.

To correctly capture logs and protect them by constant timer preemptions, both log buffer writing and protection are required to execute in {\em atomic contexts}.
%
Otherwise, the preemption not only disrupts the deadline but causes fault (\eg by writing logs to a just-protected buffer before fetching a new current buffer).
%
To this end, \codename enforces each core to acquire a lock before every log write.
%
On timer interruption, the timer thread acquires those locks before protection. 
%
Since the lock is released after every write, this timer thread acquires it within a tiny delay (less than a hundred CPU cycles in our experiments).

% Importantly, 
\codename forcibly regulates $\epsilon$ (the time between the timer thread invocation and protection) to a small value.
%
% Otherwise, adversaries may significantly extend $\epsilon$~(\eg raising spurious interrupts~\cite{lee2021exprace} to avoid the timer thread in the kernel from being scheduled).
Otherwise, adversaries may significantly extend $\epsilon$ to corrupt the protection deadline.
%
This property is regulated by (a) prioritizing the timer interrupt kernel thread and (b) enforcing the aforementioned atomic execution of the log protection.
% , which disallows task preemptions or other IRQs during log buffer permission switching.
%
The former prevents the timer thread from being delayed by other interrupts (\eg by raising spurious interrupts~\cite{lee2021exprace}). 
%
% This prevents attackers from raising spurious interrupts~\cite{lee2021exprace} to hinder the timer thread from being scheduled.
%
The latter ensures the permission switch procedure cannot be extended by other task preemptions or IRQs.

% %
% Therefore, despite potential adversarial tactics (during system exploitation), including invoking numerous interrupts~\cite{lee2021exprace} or overwhelming the buffer with excessive log events~\cite{riccardo2020kennylogging}, all captured logs are enforced to be generated and protected in memory within the real-time deadline.
% % 

% 
% \PP{Power-off log persistence guarantee.}
% \PP{Eventual pre-shutdown log persistence.}
\PP{Fast buffer consumption with eventual persistence.}
%
\hd consumes the protected buffer (\ie persists its contents to disk) and then returns the buffer into the kernel buffer pool (\ie switches its domain to the untrusted).
% 
It consumes buffers efficiently using multi-threading and {\em real-time} techniques~\cite{ahmad2022hardlog}.
% 
Since \hd might not be scheduled after OS compromise, \sm ensures all remnant buffers (in the trusted domain) are persisted before shutdown events.
% 

\hd separates its threads~(\cref{subsec:design_security_monitor}) to the consumer thread for log consumption and the manager thread for log persistence and admin task response.
%
By doing so, heavy I/O and network jobs are dispatched to the manager thread.
% 
In addition, the consumer thread is prioritized by (an honest) OS over other threads.
% 
Moreover, all hardware interrupts, except for the protection scheme timer, are disabled by the OS during the thread's execution.
%

%
\hd requests the monitor to persist the consumed logs through the debloated driver.
%
% Since \hd is a userspace daemon (unlike prior work~\cite{varun2023omnilog}), it cannot directly invoke I/O operations.
Since \hd is at userspace, it cannot directly issue I/O operations.
% 
% A userspace process cannot call \smc either to communicate with \sm.
% 
Hence, the manager thread executes an {\em ioctl} system call as a proxy, which then invokes \smc.
% 
This is just a notification mechanism, all message passing between \sm and \hd is done using a reserved {\em communication buffer} within \hd's memory.
% 
When there are no logs, \hd goes to sleep.
% 

%
% \hd separates its log {\em consumer thread} with the other {\em manager thread} .
%
% This ensures heavy jobs~(\ie I/O and network) are dispatched, allowing log buffers to be consumed and returned to \domu in time.
% %
% As such, the manager thread then is dispatched to perform heavy log persistence tasks (issuing I/O jobs through \sm's debloated driver interface in~\cref{subsec:design_security_monitor}) concurrently.

% %
% Note that the manager thread should request \sm to execute I/O tasks, by asking the OS to execute \textcode{SMC}. 
% %
% The \textcode{SMC} service command information is encoded into {\em ComBuf} (\cref{subsec:design_security_monitor}), so that a malicious OS cannot impersonate \hd to issue a fake request (as it cannot assess \domhd).
% %
% In addition, to quickly consume logs, \codename guarantees the real-time preemption~\cite{ahmad2022hardlog} of \hd's consumer thread, prioritizing its execution.
% % 
% Moreover, all hardware interrupts, except for the protection scheme timer, are disabled by the OS during the thread's execution.
% %

% Besides \hd's memory domain (\domhd) is isolated from the OS,
% its micro-architecture (cache, TLB) is disallowed to be shared with other CPU cores~\cite{zhang2023shelter,cerdeira2022rezone}.
% %
% Thus, a compromised OS on other CPUs cannot (a) bypass GPT checks to access \domhd via exploiting shared GPT entries in TLB~\cite{zhang2023shelter} or (b) slow down the log consumption by evicting \hd's cache lines~\cite{ahmad2022hardlog}.
% %
% The CPU affinity of \hd is also configured to a dedicated core to avoid frequent micro-architectural refreshing.
% %

%
The monitor intercepts power management operations to ensure all protected logs are persisted.
%
% Since a log buffer in \domhd is consumed by \hd for asynchronous persistence in the background.
% %
% An adversary may kill \hd and launch a power-off attack after the OS compromise, causing all logs not yet persisted to be lost, harming the availability of logs.
%
In particular, it intercepts the Power State Coordination Interface (PSCI) and issues an I/O command to persist all protected logs forcibly before power events~\cite{varun2023omnilog,ahmad2022hardlog}.
%

% (\circlewhite{1}--\circlewhite{3}, \circlered{1}--\circlered{\Aa{2}{b}}, \circleblue{A}--\circleblue{B})
\cref{fig:workflow} illustrates the procedure.
%
The consumer thread consumes logs in the protected buffer (\circlewhite{1}--\circlewhite{2}), and asks the monitor (\circlewhite{A}--\circleblack{A}) to edit the untrusted domain's permission to return the buffer (\circlered{1}--\circlered{\Aa{2}{b}}).
%
Meanwhile, the manager thread requests \sm to persist them into secure storage via the debloated driver interface (\circleblue{A}--\circleblue{B}).
%
Finally, before power events, \sm issues an I/O command via its debloated driver to force all protected logs to be persisted to the storage.

% \adil{Important: what happens when buffers are full? How many buffers do you have?}\chuqi{explained in Unified log protection + Unprolongable deadline property guarantee}
% \chuqi{todo: refine place to introduce. hardlog explains that in "Bounded thread execution"}
% \adil{What about through side-channel interference (e.g., cache pollution)? Do you mention in the threat model that side-channels are out-of-scope?}\chuqi{todo: add to out-of-scope}

% \adil{IMPORTANT: Is the buffer per-core? Is the timer per-core?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Secure Daemon with Log Management Tasks}
% \subsection{Remote Log Management}
% \subsection{Protected Remote Log Management Daemon}
\subsection{Secure Delegated Remote Log Management}
\label{subsec:design_daemon}
%

\codename empowers \hd to securely support remote log management tasks, such as retrieval, prior to OS compromise.
%
After compromise, the integrity of any completed management task is ensured, and the OS can only prevent new task completion~(\eg not schedule \hd).
% 
To achieve such guarantees, \hd sets up a secure channel to a remote administrator, using provisioned cryptographic secrets, over a sanitized OS-delegated network transport.
% 
% Then, its network service is transparently delegated to the OS but securely interposed by \sm.

% \PP{Offline daemon construction and secret provision}
\vspace{-0.2cm}
\subsubsection{\textbf{Daemon secret establishment.}}
% 
% Prior to deployment, a developer or administrator must construct a daemon program and provision a cryptographic secret for secure communication.
%
During machine provision (\cref{subsec:system_model}), the administrator installs the log daemon \hd, and sets up cryptographic secrets for runtime secure communication.
% 

%
% In particular, the daemon is constructed based on the requirements of the protected process~(\cref{subsec:design_security_monitor}) and the enterprise task specifications~(\eg support log filtration tasks based on process identifier~\cite{ahmad2022hardlog}).
% 
To ensure secure communication, the administrator provisions a key pair.
%
The secret portion of the key is installed on the protected disk, while the public portion is kept by administrators for later authentications.
% 
% \sout{They will provision the secret portion of the key within the protected storage disk, while keeping the public portion for later authentication}.
% 
Besides that, admins also install their own public key into the protected disk to ensure a {\em two-way} authenticated and secure channel can be created.
% 
Since the protected storage disk can only be accessed by the monitor,
% 
during \hd loading, \sm securely installs the provisioned keys within a reserved region of \hd.
% 
Thus, the key remains protected from the untrusted OS.
% 
% \chuqic{Note that such machine provisioning is common practice in enterprise management, following the Intel Active Management Technology (AMT)~\cite{intel-amt})}.

% \PP{Cryptographic secret provisioning}
% \PP{Provisioned secret-based authenticated channel}
% 


% In addition, the administrator will, at this time, also install the \sm and \hd binaries into the protected disk.
% % 
% Specifically, \hd is compiled and packaged with all required libraries~(\eg \textcode{libc}) in a statically-linked manner.
% % 
% This avoids insecure code-sharing with OS-controlled libraries and simplifies its load and measurement (\cref{subsec:design_security_monitor}).
% %

% 
% Moreover, \hd's specialized exception vector table is compiled.
% %
% This later is used by \sm to transparently and securely interpose on \hd during context switches (\cref{subsec:design_daemon}).



% \PP{Secure daemon-monitor interface establishment}
% % 
% Finally, \sm also allocates a tiny region within \hd's address space, {\em ComBuf}, which is reserved for secure bi-directional communication between \sm and \hd.
% % 
% Please refer to~\adil{refer} to understand how this region is utilized to securely ensure remote log management.\adil{change.}
% % 
\vspace{-0.2cm}
\subsubsection{\textbf{Secure channel over sanitized delegated network.}}
%
\codename sends and receives packets through OS network interfaces, but ensures packets are secured end-to-end between \hd and the administrator.
%
It is ensured by the Transport Layer Security (TLS) protocol and the key pair provisioned.
%
Therefore, adversaries cannot impersonate the remote admin (\eg forge and issue log deletion requests and responses).
% 
The remaining paragraphs illustrate how network system calls from \hd are supported and sanitized.
% 

\sm interposes \hd's network service system call invocations and returns (\ie context switches) to perform secure domain transitions.
%
The interposition is enforced through \hd's specialized exception vector table, which is transparent to the OS (\cref{subsubsec:daemon_execution}).
%
As such, \hd's execution context is securely saved and managed by \sm.
%
At syscall invocations, before switching the memory-view to the untrusted domain to enter the OS, syscall pointer parameters are redirected to a shared buffer that is accessible in the OS.
%
Otherwise, the OS cannot access \hd's memory buffer pointed by the syscall parameters (in the trusted domain).
%

Once the syscall returns, the monitor sanitizes the return values before resuming \hd.
% 
In particular, to prevent pointer-based IAGO attacks~\cite{stephen2013iago}, \sm ensures that no pointer is returned for a region that belongs to \hd's domain.
% 
Moreover, \sm copies the packet data from the shared buffer into \hd's buffer.
%
Then, \sm transits to the trusted domain (activating \hd's memory view), restores the context, and enforces its maintained \hd page table and vector table.
%
Finally, \sm transits the CPU execution to \hd.

\cref{fig:workflow} (\circlewhite{X}--\circlewhite{Z}, \circlewhite{A}--\circlewhite{B}, \circleblack{A}--\circleblack{B}) illustrates the interposed context switch.
%
Whenever \hd requests network services (\circlewhite{X}, \circlewhite{Z}), it traps to \sm (\circlewhite{A}--\circleblack{A}) by its customized exception vector table.
%
\sm then saves its context, redirects pointer parameters, transits to the untrusted domain (\circlered{1}), and then exits to the OS (\circleblack{B}).
%
Whenever the OS finishes the service, \sm interposes the return (\circleblack{A}) and performs the context switch on the OS' behalf.
%
It restores the saved contexts, enables \hd's domain (\circlered{1}), enforces its page and vector table, and directly returns to \hd's execution context (\circlewhite{B}).


% \begin{table}[H]
%     \centering
%     \caption{\codename user interfaces.}
%     \label{tab:user_interface}
%     \setlength{\aboverulesep}{0pt}
%     \setlength{\belowrulesep}{0pt}
%     \begin{adjustbox}{width=0.5\textwidth}
%     \begin{tabular}{@{}l|l@{}}
%       \specialrule{0.1em}{\aboverulesep}{0pt}
%       \textbf{Name} & \textbf{Description} \\
%       \specialrule{0.05em}{0pt}{\belowrulesep}
%       \specialrule{0.05em}{1pt}{\belowrulesep}
%       \texttt{hhkr\_register\_obs()}  & Register an observability type and its buffer pool. \\
%       \texttt{hhkr\_write\_obs\_buf()}           & Write to the current buffer of a given observability type.           \\
%       \texttt{hhkr\_get\_obs\_buf()}             & Get the current buffer of a given observability type.           \\
%       \texttt{hhkr\_sec\_obs\_buf()}             & Secure the current buffer of a given observability type.   \\
%       \specialrule{0.1em}{0pt}{\belowrulesep}
%     \end{tabular}    
%     \end{adjustbox}
%   \end{table}


==> tex/design-old.tex <==
\section{\codename Design}
\label{sec:design}
%

\adil{Intro.\\
C1: creating a high-assurance environment based on proposed strategies,\\
C2: ensuring short, real-time deadlines using memory protection mechanisms,\\
C3: 
}

\subsection{Offline System Bootstrap}
\label{subsec:design_offline}
% 

Prior to runtime initialization, the system administrator completes two tasks.
% 
First, they synthesize a debloated driver template for their system using our provided recorder tool.
% 
This template is used by \sm for reading and writing data to the disk at runtime (\cref{subsec:design_security_monitor}).
% 
Second, they install a cryptographic secret into the protected log storage disk.
% 
This is used for secure communication between \hd and the remote administrator (\cref{subsec:design_daemon}).
% 

\PP{Debloated driver template synthesis.}
%
\codename provides an offline tool to synthesize a debloated storage template prior 
to system bootstrap, which is later instantiated into \sm during its initialization. 
%
This is done by using record-and-replay mechanisms~\cite{wang2022rttee,guo2022driverlet} for storage drives (\eg SATA, USB, etc), as a one-time effort.

% 
Our record-and-replay tool considers a storage device as a finite state machine (FSM).
%
Hence, the operations of a driver 
are distilled into a sequence of {\em driver-device} interactions, each of which is a FSM transition.
% 
These interactions remain consistent irrespective of the I/O task payload variations~\cite{guo2022driverlet} to be recorded into a {\em template}.
%
In particular, during the recording phase, we issue sample I/O jobs to log storage and templatize the following interactions (detailed in \cref{sec:impl}):
% 
(1) the sequences and content of Memory-mapped I/O (MMIO) write operations to the log storage, 
(2) the allocation of direct-memory-access (DMA) buffers for the log storage, and 
(3) interrupt request (IRQ) numbers invoked by the log storage, along with the completion status.
%
The template is then installed into \sm's binary.
%
Note that the recording phase is a one-time effort from an administrator's perspective.

\PP{Cryptographic secret and binary provisioning}
% \PP{Log storage disk preparation}
% 
The administrator will create a cryptographic secret key pair. 
% 
They will install the secret portion of the key into the protected storage disk, while keeping the public portion for future secure communication (\cref{subsec:design_daemon}).
% 
The protected storage disk will only ever be accessed by \sm (\cref{subsec:design_security_monitor}); hence, this key is safe.
% 
In addition, the administrator will, at this time, also install the \sm and \hd binaries into the protected disk.
% 
Specifically, \hd is compiled and packaged with all required libraries~(\eg \textcode{libc}) in a statically-linked manner.
% 
This avoids insecure code-sharing with OS-controlled libraries and simplifies its load and measurement (\cref{subsec:design_security_monitor}).
%
Moreover, \hd's specialized exception vector table is compiled.
%
This later is used by \sm to transparently and securely interpose on \hd during context switches (\cref{subsec:design_daemon}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{fig/workflow.pdf}
%     % \vspace*{-0.7cm}
%     \caption{\codename memory layout, memory views, and workflow. \codename Monitor (\sm \boxsm) is the security monitor.
%     %
%     \codename Daemon (\hd~\boxhd) is the secure log daemon.
%     %
%     All trusted components are denoted as {\bf TR} (\boxsm~\boxhd). 
%     %
%     Other parts are untrusted (denoted as {\bf UT}~\boxns).
%     %
%     \sm maintains and configures two GPTs ({\sc GPTut} and {\sc GPTtr}) in different CPU modes, which isolates the memory view of the secure environment from the untrusted OS.
%     } 
%     \label{fig:workflow}
%     %\vspace{-0.15cm}
% \end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/workflow_short.pdf}
    % \vspace*{-0.7cm}
    \caption{
    \codename workflow and memory protection domains.
    %
    \sm (\boxsm\ \domsm) and \hd (\boxhd\ \domhd) are trusted components, while the host OS and all its applications (\boxns\ \domu) are untrusted.
    } 
    \label{fig:workflow}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Secure Environment Setup and Bootstrap}
% \subsection{Secure Environment Intialization}
\subsection{Secure High-Assurance Environment Setup}
\label{subsec:design_security_monitor}

% \codename's secure environment is set by the administrator before the system bootstrap.
% %
% The administrator is responsible for provisioning a pair of keys to enable the secure authentication channel~\cite{ahmad2022hardlog,varun2023omnilog} for remote communication.
% %
% The public key is always set up inside \sm and loaded during secure boot, while the administrator keeps the private key.
% %
% In addition, apart from normal system devices (\eg filesystem and storage), a {\em secondary log storage device} is connected to the host dedicated to log persistence.
%
% A debloated driver for this log storage 

% \codename is set up by the administrator prior to system bootstrap (\cref{subsec:threat_model}).
% %
% The cryptographic key is set up inside \sm's binary and loaded during the secure boot.
% %
% Additionally, a protected debloated driver for \codename's log storage device is synthesized offline into \sm for secure log persistence.
% %

% During system boot, \codename then verifies \sm initialization and protection mechanisms setup, reserves the host memory layout to configure memory permissions in \sm, and finally boots and starts the OS.
\codename first initialize \sm to isolate system resources (memory, device) to maintain its secure environment.
%
After setting up its secure environment, the OS is booted to start the protected observability software stack.

%%
% \PP{Offline debloated driver template synthesis.}
% %
% \codename provides an offline tool to synthesize a debloated storage template prior 
% to system bootstrap, which is later instantiated into \sm during its initialization. 
% %
% This is done by using record-and-replay mechanisms~\cite{wang2022rttee,guo2022driverlet} for storage drives (\eg SATA, USB, etc), as a one-time effort.

% % 
% Our record-and-replay tool considers a storage device as a finite state machine (FSM).
% %
% Hence, the operations of a driver 
% are distilled into a sequence of {\em driver-device} interactions, each of which is a FSM transition.
% % 
% These interactions remain consistent irrespective of the I/O task payload variations~\cite{guo2022driverlet} to be recorded into a {\em template}.
% %
% In particular, during the recording phase, we issue sample I/O jobs to log storage and templatize the following interactions (detailed in \cref{sec:impl}):
% % 
% (1) the sequences and content of Memory-mapped I/O (MMIO) write operations to the log storage, 
% (2) the allocation of direct-memory-access (DMA) buffers for the log storage, and 
% (3) interrupt request (IRQ) numbers invoked by the log storage, along with the completion status.
% %
% The template is then installed into \sm's binary.
% %
% Note that the recording phase is a one-time effort from an administrator's perspective.

% \PP{System memory layout reservation}
% \PP{System memory domains creation}
\PP{Memory protection domain enforcement}
%
\sm assigns three memory protection domains: one for its own reserved memory regions (\domsm), one for \hd's regions (\domhd), and one for regions belonging to the remaining untrusted components---the host OS, all its applications, and the log capturer (\domu).
% 
The paragraphs below explain how these domains are isolated and securely transitioned.
% 

% \sm creates two isolated memory protection domains: trusted (\domt) and untrusted (\domu).
% 
% {\domt} contains all reserved memory regions where \sm resides,  alongside its permission switch primitives (\ie GPT configurations) and the aforementioned debloated driver.
% % 
% It also contains the reserved physical address space for \hd, including its binary sections and execution stacks.
% % 
% In contrast, \domu holds the regions for the untrusted system components (\ie host OS and all its applications).
% % 
% The paragraphs below explain how these domains are isolated and securely transitioned.

% {\bf{\Aa{D}{T}\xspace}} contains all reserved memory regions of \sm and \hd, while {\bf{\Aa{D}{UT}\xspace}} holds the regions for the untrusted system components (\ie host OS and all its applications).
% % 

% ~\cite{sridhara2023acai,zhang2023shelter,hof2022blackbox}

\sm prevents the malicious CPU (MMU) and device (DMA) access to trusted domains (\domsm and \domhd) using GPT and the System Memory Management Unit (SMMU), respectively. 
% 
To isolate CPU memory access to the trusted domains, \sm creates (and maintains) two GPTs within its domain \domsm~\cite{sridhara2023acai,zhang2023shelter,hof2022blackbox}: one where regions for untrusted components (\domu) are marked accessible and another where \hd's regions (\domhd) are marked accessible.
%
\sm regions are also marked accessible to both GPTs, allowing domains to call \sm for a service~(\eg log protection or retrieval).
% 
This is secure since, within both GPTs, \sm regions are marked as {\em root} (\cref{sec:arm_background}), which allows their access to \domsm in the EL3 CPU execution mode {\em only}.
% 
% This allows \sm to modulate memory views, ensuring that CPUs can only access their dedicated memory in specific execution modes.
%
Moreover, \sm configures SMMU to limit device memory addressing~\cite{varun2023omnilog,sridhara2023acai}.
%
The SMMU configuration interfaces (\eg control registers and stream tables) are also protected within \domsm (by \domu's GPT restriction)~\cite{sridhara2023acai}.
% 


% \sm also interposes all domain transitions to ensure correctness.
% % 



% \sm divides the system into 4 memory regions (the left table in~\cref{fig:workflow}).
% %
% \begin{enumerate}[leftmargin=*,label=\textbullet]
%     %
%     % An untrusted OS can only access this region at runtime.

%     \item
%     {\bf{\Aa{M}{\sm}\xspace}} is where \sm resides,  alongside its permission switch primitives (\ie GPT configurations) and the aforementioned debloated driver.
%     % 
    
%     % , and other platform-generic security services~\cite{atf}.
    
%     \item
%     {\bf{\Aa{M}{\hd}\xspace}} is the reserved physical address space for \hd, including its binary sections and execution stacks.
    
%     \item{\bf{\textsc{Mbufpool}\xspace}} is an in-kernel buffer pool designated for log capture and runtime permission switch.

%     \item
%     {\bf{\textsc{Mut}\xspace}} is the region for the untrusted system domains (\ie host OS, all its applications, and normal driver interfaces).

% \end{enumerate}

% \adil{4 memory regions and only 2 GPTs is confusing.}
% \chuqi{Mut is Dut, Mhkd and Mhkm are Dt, Mbufpool are dynamically between Dut and Dt?}

% Once setting up the system layout, \sm configures memory protection mechanisms to isolate the secure environment from the OS (explained in the following).

% \PP{Memory-view partition and isolation.}
% \PP{Protected memory region initialization.}
% \PP{Reserved memory region protection}
% % 
% \sm configures GPT and System Memory Management Unit (SMMU) to isolate the secure environment memory regions from untrusted domains CPU and device DMA access, respectively.

%
% To isolate untrusted OS' CPU memory access to the secure environment, \sm creates and maintains two GPTs~\cite{sridhara2023acai,zhang2023shelter,hof2022blackbox}: one for the untrusted system ({\sc GPTut}) and the other for the trusted components ({\sc GPTtr}).
% %
% This allows \sm to modulate memory views, ensuring that CPUs can only access their dedicated memory in specific execution modes.
% %

As noted above, both \domu and \domhd can call \sm for a service. 
% 
This is achieved using an \textcode{SMC}~(\cref{sec:arm_background}).
% 
A special \textcode{SMC} is also used to transition between domains (\eg when the OS schedules \hd).
% 
In such calls, \sm swaps the GPT pointers in the \textcode{GPTBR\_EL3} register and returns to the target domain.
% 
Please refer to \cref{subsec:design_daemon} for additional details.
% 

% When a CPU operates in untrusted domains (OS and applications), {\sc GPTut} {\em always} restricts its permissions to the secure environment, confining it to the {\sc Mut} (see memory views in \cref{fig:workflow}).
% %
% \sm, during runtime, performs security checks and changes the activated GPT for CPU context switches between domains (\cref{subsec:design_daemon}).
% %
% \adil{Chuqi, can you explain this better?}

% Apart from confining CPUs' memory permissions by GPT checks during MMU walks, \sm also addresses DMA access configuration
%  for devices to prevent DMA attacks.
% %
% To do so, \sm configures SMMU to limit device memory permissions~\cite{varun2023omnilog,sridhara2023acai}.
% %
% Moreover, the SMMU configuration interfaces (\eg control registers and stream tables) are then protected in \sm~\cite{sridhara2023acai} 
% by {\sc GPTut} (\ie the untrusted domains can not tamper with SMMU configuration).
%
% This concept aligns with common practices~\cite{hofmann2013inktag,hof2022blackbox,zhang2023shelter,sridhara2023acai} that leverage permission primitives for physical memory space access control

% \adil{why do we need this sentence? Avoid talking about existing work in design.}\chuqi{removed}
%
% By doing so, our system is an extension of the CCA Realm world, which is orthogonal to the original purpose and doesn't require any modification of its own codebase (discussed in APPEN.X)~\cite{sridhara2023acai,zhang2023shelter}.
% \adil{Is it really an extension? It's not clear how/why at this point. Clarify.}\chuqi{removed}

\PP{Log storage disk initialization.}
%
\sm sets-up the debloated driver template during initialization to enable communication with the log storage disk.
%
Specifically, the driver's MMIO regions (which are fixed physical addresses) and allocated DMA buffers are only mapped to \domsm.
% 
Recall that this region is protected by GPT and SMMU, hence the untrusted OS cannot manipulate protected driver interfaces.
% 
To ensure interrupts from the log storage disk are routed to the protected driver only, \sm updates the IRQ table in the EL3 interrupt management framework~\cite{irqroute}.
% 
At runtime, \sm replays the template with dynamic parameters (\eg MMIO control sequences to write disk sectors to persist logs to disk).
%

\PP{Collaborative userspace log daemon installation}
% 
After the OS boots up, one of its initial tasks is to install \hd as a {\em protected multi-threaded user-space process} under its management.
% 
This is securely completed in collaboration with \sm as we describe next, and it can be completed with minor changes to the kernel using a loadable module~(\adil{refer}).
% 

% 
\sm retrieves the \hd binary from the protected disk and sends it to the OS for installation.
% 
\sm can simply install the binary itself, but this would unnecessarily bloat and complex \sm's TCB.
% 
Instead, OS loads the process and sets up its virtual space mapping to an OS-allocated region during loading, \sm verifies the correct layout of its binary.
% 
This is similar to how remote users attest that an SGX enclave~\cite{mckeen2013sgx} is correctly installed by the OS.
%
% 
To prevent time-of-check-to-time-of-use (TOCTOU) attacks, the OS-allocated region is protected in \domhd once the page is set up (using \sm's domain enforcement) before verification.
% 
If verification fails, the OS is considered malicious, and logging is halted with a warning log message.
%
OS also pre-allocates and sets up the execution stacks for \hd thread initialization, and calls \sm to verify and protect their stacks in \domhd.

%
Once installed, \sm maintains the page tables of \hd.
%
The initial page table mappings are provided by the OS, but are also verified using the process mentioned in the last paragraph.
% 
After verification, \hd's pages are {\em pinned} in memory. 
%
As its page table is maintained inside \domsm, the OS cannot make any changes to the verified mappings to perform page remapping attacks~\cite{hofmann2013inktag}.
% 
This is acceptable since \hd only requires a small amount of reserved memory~(less than 16MB in our implementation).
%

\PP{Secure daemon-monitor interface establishment}
% 
Finally, \sm also allocates a tiny region within \hd's address space, {\em ComBuf}, which is reserved for secure bi-directional communication between \sm and \hd.
% 
Please refer to~\adil{refer} to understand how this region is utilized to securely ensure remote log management.\adil{change.}
% 


% 
% The OS allocates a region of memory for \hd.
% % 
% \sm leverages its memory domain enforcement mechanisms (previous heading) to protect this region in \domhd.
% % 
% \sm then retrieves the \hd binary from the protected disk, and securely loads the binary pages into the protected region.
% 

% \sm interposes \hd's binary load (through a specialized kernel module) during initialization, to attest to its correctness and protect it.
% % 
% During the virtual address space setup, \sm creates and maintains the page table of \hd, mapping its address space to the reserved region \Aa{M}{\hd}.
% %
% To prevent time-of-check-to-time-of-use (TOCTOU) attacks, each page mapping is protected and fixed before verification.
% %
% Then, \sm verifies each page using an SHA-256 cryptographic hash~(like SGX enclaves~\cite{mckeen2013sgx}) and compares the final measured hash against a pre-determined value.
% % 
% If the comparison is false, the OS is considered malicious, and logging is halted with a warning log message.
% % 
% %
% After verification, \hd's pages are {\em pinned} in memory. 
% %
% As its page table is maintained inside \domsm, the OS cannot make any changes to the verified mappings to perform page remapping attacks~\cite{hofmann2013inktag}.
% % 
% This prepaging is acceptable since \hd does not require a significant amount of memory or dynamic memory updates.

% \PP{Log buffer pool and timer specification.}
% %
% A dynamic buffer pool is maintained for the capturer, wherein the permissions of each buffer are switched based on a timer-defined real-time deadline.
% %
% %
% \codename promptly pops the {\em current log buffer} from the pool for protection (\cref{subsec:design_realtime_deadline}), and concurrently consumes the buffer in the background \hd, subsequently placing it back to the pool (\cref{subsec:design_daemon}).
% %
% \codename's hardware timer is activated once the observability capturer is enabled.
% %
% Since the OS is initially benign after the secure boot, the timer is correctly deployed before the OS compromise ($t_c$).

% \chuqi{To be shorten: record-and-replay and storage initialization filled too much space}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Deadline-Enforced Log Protection}
\label{subsec:design_realtime_deadline}

% \codename assigns each log buffer a protection window of $T_p + \epsilon$, and ensures $\epsilon$ (\cref{subsec:overview_inmemory_observability_protection}) to be small and regular to enforce the real-time deadline.
% %
% Otherwise, adversaries may delay the deadline by prolonging $\epsilon$, obtaining a larger window to tamper with logs after compromising the OS~\cite{riccardo2020kennylogging}.

%
\codename enforces log protection {\em from its capture to its persistence} to maintain log integrity and availability.
%
Different logs are collected in a unified location to standardize the protection window.
%
A hardware timer then ensures the collected logs are protected in memory within the configured delay.
%
Finally, the protected logs are securely persisted into the protected disk to guarantee availability.
%

% Without the log persistence guarantee, the in-memory protection would be futile as logs can be dropped after the system powers off.
%
% \adil{Please shorten intro into 3-4 lines (high-level).}
% \chuqi{check}

% \PP{Log buffer pool and timer specification.}
%

% 
% %

% \adil{Merge this and the next heading into one heading that describes (a) how the kernel keeps a log buffer pool and (b) how all logs are collected within the buffers. You should shortly mention eBPF here, since its part of your figure, and its not obvious how you collect logs in a unified manner otherwise. Move the timer aspecs into the "hardware timer-..." heading.}


% \PP{Unified log capture in singular buffers.}
% \PP{Log buffer pool-based unified capture.}
\PP{Unified log collection in kernel buffer pools.}
%
Capturing logs at different locations (\eg network drivers, applications) in an ad-hoc manner and protecting them can increase protection delay.
% 
\codename avoids this by unified capturing logs within the kernel before protection~(\circleblack{1}--\circleblack{2} in~\cref{fig:workflow}).
% 

\codename requires two aspects for unification: (a) a central region (buffer) to hold logs and (b) a mechanism to generate the captured events as logs to that region.
% 

% 
To create a central region, \codename allocates a {\em pool of per-core} buffers within the kernel observability generator's memory.
% 
Logs are always written to the {\em current} buffer within the pool.
%
A pool of (at least two) buffers is required, because \codename dynamically switches the {\em current} buffer's domain for protection (as explained in the next heading).
%
Hence, there should be always an available buffer to serve as the {\em current}.
% 
The size of the buffers is administrator-controlled.
% 
If the buffer becomes full, very rare in honest scenarios based on proper configuration in our evaluation~(XX) and prior work~\cite{varun2023omnilog}, the generator waits for a buffer to be consumed and returned.
% 
This prevents attackers from having their attack trace overwritten even if they generate many spurious logs from userspace before compromise.
% 

% For generating logs, our implementation leverages eBPF~\cite{ebpf,tracee}~(more details in~\cref{sec:impl}).
% % 
% Note that this can be easily ported to other tools like KLogger~\cite{yoav2007klogger} and can support extra log sources through diverse probes (discussed in~\chuqi{X}).
% % 

\codename collects the logs generated by applications using the extended Berkeley Packet Filter~(eBPF)~\cite{ebpf}~(\circleblack{1}), which is widely-used in prior work~\cite{agman2021bpfroid, minna2023sok}.
% 
A challenge in capturing logs from applications is locating and automatically intercepting the routines where logs are generated.
% 
This is addressed by performing {\em contextual tracking} of file system calls.
% 
Specifically, applications leverage the file system to write logs. 
% 
Thus, the generator records {\em write-related} syscalls and extracts their file paths in kernel runtime structures (\eg \textcode{dentry} from \textcode{vfsmount}) to match them with administrator-defined log file paths (\eg \textcode{/var/app.log})~\cite{tracee}.
% 
For relevant log file writes, \codename then extracts the content using an eBPF probe.
% 

In contrast to application logs, \codename generates and collect logs from network and system calls using eBPF~(\circleblack{2}).
% , \codename leverages the extended Berkeley Packet Filter~(eBPF)~\cite{ebpf}, like prior work~\cite{agman2021bpfroid, minna2023sok}. 
%
Specifically, \codename injects BPF programs into kernel tracepoints to attach all 436 system calls and socket-related events.
%
\codename follows Linux Auditd's format~\cite{auditd} to generate system call log entries, which includes parameters, return values, and other fields (\eg process identifiers and timestamps).
% 
For network traffic logging, \codename logs IP, ports, and other packet data from the kernel socket structure for network traffic.
% 



% A buffer pool is maintained for the capturer, wherein the permissions of each buffer are switched between {\domu and \domhd} dynamically.
% %
% The capturer records multi-layer observability logs from the kernel.
% %
% To unify their protection window, \codename captures all logs within the same kernel buffer before protection.
% 

% \chuqi{leave to implementations}
% % 



% Our implementation leverages eBPF~\cite{ebpf,tracee} for observability capturer~(more details in~\cref{sec:impl}).
% % 
% Note that this can be easily ported to other tools like KLogger~\cite{yoav2007klogger} and can support extra log sources through diverse probes (discussed in~\chuqi{X}).
% \adil{(e.g., write, fwrite, fput)}\chuqi{honestly only write are typically used in app. logs. fwrite and fput are not syscalls but libc funcs.} 
% \adil{Minor: How do you correlate?}\chuqi{fixed. it's predefined by administrators}

% \adil{can you have a heading here talking about how you handle the (16?) buffers? You also need to mention that you pause execution if buffers become full.}\chuqi{fixed}

% \adil{Unprolongable is not a word. Heading is not about the guarantees, its about how you enforce them. The section heading already says "deadline".}

% Given the deadline of $T_p + \epsilon$, the $\epsilon$ is always kept small and regular for buffer protection (context switches and GPT configurations shown in~\cref{tab:prot_primitives}), 
% %
% In other words, attackers shall not prolong this deadline during system exploitation.

% \PP{Prompt timer response with no drop protection.}
\PP{Hardware timer-initiated log buffer protection.}
%
The OS deploys a hardware timer based on the administrator's configured frequency (i.e., $T_p$ as discussed in~XX) and directs a kernel thread to initiate log protection.
% 
Since the OS is initially benign after the secure boot (\cref{subsec:threat_model}), the timer is correctly deployed before the OS compromise ($t_c$).
% 
Moreover, \codename~{\em controls} the delay after the timer expires to ensure that protection is achieved within a small period ($\epsilon$).
% 
This ensures that each log's protection deadline is $T_p + \epsilon$.
% 
We explain all these aspects in the next paragraphs.

% normal latency due to timer response, context switches, and buffer permission switch.
% (\cref{subsec:overview_inmemory_observability_protection}).
%

% \codename's hardware timer is activated once the observability generator is enabled.
% %
% Since the OS is initially benign after the secure boot (\cref{subsec:threat_model}), the timer is correctly deployed before the OS compromise ($t_c$).
%

%
% In addition, log events are kept protected with no drop.
\cref{fig:workflow} illustrates log protection.
%
Once logs are captured, \codename writes them to a {\em current} buffer~(\circleblack{\Aa{3}{a}}). 
%
When a timer deadline is reached, a kernel thread calls \sm (\circleblack{\Aa{3}{b}}--\circleblack{A}) to switch the current buffer's domain from \domu to \domhd (\circlered{1}--\circlered{\Aa{2}{a}}).
%
After protection is complete, a new buffer is fetched from the pool, which becomes the new {\em current} (\circleblack{B}--\circleblack{\Aa{3}{c}}).
% 
The previous (now protected) buffer will be re-inserted to the pool after consumption~(next heading).

% \adil{explain in next heading?}
% After the protected buffer is consumed, its domain switches back to \domu to re-add to the pool~(explained in the next heading).
% %
% If all buffers are exhausted or full, the CPU context associated with the log event is paused to prevent log drop~\cite{ahmad2022hardlog}, until a protected buffer's permission is returned by \hd.

It is essential to regulate $\epsilon$ (i.e., the time between kernel thread invocation and protection) to a small value.
%
Otherwise, adversaries may significantly extend $\epsilon$~(e.g., raising spurious interrupts to avoid the timer thread in the kernel from being scheduled).
%
This property is enforced by (a) prioritizing the timer interrupt response kernel thread and (b) ensuring the atomic execution of the log protection, thereby disallowing task preemptions or other IRQs during the log buffer's domain (permission) switch procedure.
%
The former prevents the timer thread from being delayed by other interrupts, while the latter ensures the deadline cannot be extended by preempting or interrupting the permission switch procedure.

% %
% Therefore, despite potential adversarial tactics (during system exploitation), including invoking numerous interrupts~\cite{lee2021exprace} or overwhelming the buffer with excessive log events~\cite{riccardo2020kennylogging}, all captured logs are enforced to be generated and protected in memory within the real-time deadline.
% % 

% 
% \PP{Power-off log persistence guarantee.}
% \PP{Eventual pre-shutdown log persistence.}
\PP{Fast buffer consumption with eventual persistence.}
%
\hd is scheduled by the OS to consume the protected buffer (i.e., persists its contents to disk) and then return the buffer into the kernel buffer pool (i.e., switches its domain to \domu).
% 
\hd consumes buffers efficiently using multi-threading and {\em real-time} techniques~\cite{ahmad2022hardlog}.
% 
Since \hd might not be scheduled after OS compromise, \sm ensures that all remnant buffers (in \domhd) are persisted before any shutdown event.
% 

\hd dedicates one of its threads, the {\em consumer thread}, for log persistence.
% 
This thread is prioritized by the OS over the other {\em manager thread} (which is used for remote retrieval in~\cref{subsec:design_daemon}).
% 
Moreover, all hardware interrupts, except for the protection scheme timer, are disabled by the OS during the thread's execution.
%
Since \hd is user-space (unlike prior work daemons~\cite{varun2023omnilog}), it cannot directly invoke I/O operations.
% 
Hence, its consumer thread uses the secure daemon-monitor interface~(XX) to send persistence requests.
% 
If there are no logs to be consumed, \hd sleeps and yields the core.

%
% \hd separates its log {\em consumer thread} with the other {\em manager thread} .
%
% This ensures heavy jobs~(\ie I/O and network) are dispatched, allowing log buffers to be consumed and returned to \domu in time.
% %
% As such, the manager thread then is dispatched to perform heavy log persistence tasks (issuing I/O jobs through \sm's debloated driver interface in~\cref{subsec:design_security_monitor}) concurrently.

% %
% Note that the manager thread should request \sm to execute I/O tasks, by asking the OS to execute \textcode{SMC}. 
% %
% The \textcode{SMC} service command information is encoded into {\em ComBuf} (\cref{subsec:design_security_monitor}), so that a malicious OS cannot impersonate \hd to issue a fake request (as it cannot assess \domhd).
% %
% In addition, to quickly consume logs, \codename guarantees the real-time preemption~\cite{ahmad2022hardlog} of \hd's consumer thread, prioritizing its execution.
% % 
% Moreover, all hardware interrupts, except for the protection scheme timer, are disabled by the OS during the thread's execution.
% %

% Besides \hd's memory domain (\domhd) is isolated from the OS,
% its micro-architecture (cache, TLB) is disallowed to be shared with other CPU cores~\cite{zhang2023shelter,cerdeira2022rezone}.
% %
% Thus, a compromised OS on other CPUs cannot (a) bypass GPT checks to access \domhd via exploiting shared GPT entries in TLB~\cite{zhang2023shelter} or (b) slow down the log consumption by evicting \hd's cache lines~\cite{ahmad2022hardlog}.
% %
% The CPU affinity of \hd is also configured to a dedicated core to avoid frequent micro-architectural refreshing.
% %

%
\codename intercepts power management operations to ensure protected logs are persisted.
%
% Since a log buffer in \domhd is consumed by \hd for asynchronous persistence in the background.
% %
% An adversary may kill \hd and launch a power-off attack after the OS compromise, causing all logs not yet persisted to be lost, harming the availability of logs.
%
In particular, \sm intercepts the Power State Coordination Interface (PSCI) and issues an I/O command to persist all protected logs before power events forcibly~\cite{varun2023omnilog,ahmad2022hardlog}.
%


\cref{fig:workflow} (\circlewhite{1}--\circlewhite{3}, \circlered{1}--\circlered{\Aa{2}{b}}, \circleblue{A}--\circleblue{B}) illustrates the procedure.
%
The {\em consumer thread} consumes logs from the protected buffer to its internal memory (\circlewhite{1}--\circlewhite{2}) and asks \sm (\circlewhite{A}--\circleblack{A}) to edit \domu's GPT to return the buffer (\circlered{1}--\circlered{\Aa{2}{b}}).
%
Meanwhile, the {\em manager thread} then manages logs, requesting \sm to persist them into secure storage via the debloated driver interface (\circleblue{A}--\circleblue{B}).
%
Finally, before power events, \sm issues an I/O command via its debloated driver (\circleblue{A}--\circleblue{B}) to force all protected logs to be persisted to the storage.

% \adil{Important: what happens when buffers are full? How many buffers do you have?}\chuqi{explained in Unified log protection + Unprolongable deadline property guarantee}
% \chuqi{todo: refine place to introduce. hardlog explains that in "Bounded thread execution"}
% \adil{What about through side-channel interference (e.g., cache pollution)? Do you mention in the threat model that side-channels are out-of-scope?}\chuqi{todo: add to out-of-scope}

% \adil{IMPORTANT: Is the buffer per-core? Is the timer per-core?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Secure Daemon with Log Management Tasks}
% \subsection{Remote Log Management}
% \subsection{Protected Remote Log Management Daemon}
\subsection{Secure Remote Log Management}
\label{subsec:design_daemon}
%

\codename relies on \hd to support remote log management tasks like retrieval.
%
\hd first sets up the secure channel to the admin, by using the preserved cryptographic key (\cref{subsec:design_offline}).
% 
Then, its network service is transparently delegated to the OS but securely interposed by \sm.

% To this end, simultaneous to \hd measurement and protection during initialization, \sm also creates and maintains a {\em protected page table} for \hd process using the provided virtual and physical addresses.
% %
% Before executing \hd, \sm always enforces this protected page table for address translation.


% \adil{Use the word "pinned" here while talking about HkD's pages. e.g., After verifictaion, HkD's pages are allocated and pinned during creation, and the OS is not allowed to make any changes to the verified mappings.}
% \chuqi{fixed}

% \adil{I would also mention here somewhere that HkD can be updated periodically. For instance, if the admin needs some slightly different functionality.}
% \PP{Secure channel establishment.}
%
The channel between \hd and remote administrators is encrypted by the Transport Layer Security (TLS) protocol, where the key pair is provisioned during secure boot (\cref{subsec:design_offline}).
%
Therefore, adversaries cannot impersonate the remote admin to compromise log integrity.

\noindent\textbf{Securely delegated network services.}
%
\codename securely delegates \hd's network services to the native OS.
%

\sm interposes \hd's network service system call invocations and returns (\ie context switches) to perform secure domain transitions~\cite{hofmann2013inktag,hof2022blackbox,zhang2023shelter}.
%
The interposition is enforced through \hd's specialized exception vector table (\cref{subsec:design_offline}), transparently to the OS. 
%
As such, \hd's execution context is securely saved by \sm.
%
Before switching to \domu to enter the OS, its (syscall) pointer parameters are redirected to a shared buffer which is accessible in \domu.
%
Otherwise, executing inside the OS (\domu) cannot access \hd's memory buffer pointed by the syscall parameters (inside \domhd).
%
Once the syscall returns, \sm interposes and sanitizes the return values (detailed in Appendix~\cref{appen:os_services}). 
%
Beyond correctly setting up the memory protection (activating \domhd's GPT, \cref{subsec:design_security_monitor}), \sm restores the saved context, enforces its maintained page table (\cref{subsec:design_security_monitor}) and vector table.
%
Finally, \sm transits the CPU execution to \hd to resume its execution.

\cref{fig:workflow} (\circlewhite{X}--\circlewhite{Z}, \circlewhite{A}--\circlewhite{B}, \circleblack{A}--\circleblack{B}) illustrates the interposed context switch.
%
Whenever \hd requests network services (\circlewhite{X}, \circlewhite{Z}), it traps to \sm (\circlewhite{A}--\circleblack{A}) by its customized exception vector table.
%
\sm then saves its context, redirects pointer parameters, enables \domu's GPT (\circlered{1}), and then exits to the OS (\circleblack{B}).
%
Whenever the OS finishes the service, \sm will interpose the return (\circleblack{A}) and perform the context switch on the OS' behalf.
%
It restores the saved contexts, enables \domhd's GPT, enforces its page and vector table, and directly returns to \hd's execution context (\circlewhite{B}).


% \begin{table}[H]
%     \centering
%     \caption{\codename user interfaces.}
%     \label{tab:user_interface}
%     \setlength{\aboverulesep}{0pt}
%     \setlength{\belowrulesep}{0pt}
%     \begin{adjustbox}{width=0.5\textwidth}
%     \begin{tabular}{@{}l|l@{}}
%       \specialrule{0.1em}{\aboverulesep}{0pt}
%       \textbf{Name} & \textbf{Description} \\
%       \specialrule{0.05em}{0pt}{\belowrulesep}
%       \specialrule{0.05em}{1pt}{\belowrulesep}
%       \texttt{hhkr\_register\_obs()}  & Register an observability type and its buffer pool. \\
%       \texttt{hhkr\_write\_obs\_buf()}           & Write to the current buffer of a given observability type.           \\
%       \texttt{hhkr\_get\_obs\_buf()}             & Get the current buffer of a given observability type.           \\
%       \texttt{hhkr\_sec\_obs\_buf()}             & Secure the current buffer of a given observability type.   \\
%       \specialrule{0.1em}{0pt}{\belowrulesep}
%     \end{tabular}    
%     \end{adjustbox}
%   \end{table}


==> tex/in_memory_observability_protection.tex <==
\section{In-memory Observability Protection}
\label{sec:in_memory_observability_protection}

\codename employs hardware permission-based memory access control to achieve its memory protection.

\noindent\textbf{Flexible asynchronous protection scheme.} 
The high efficiency of hardware memory protection primitive enables \codename to swiftly protect a batch of logs in memory at once.
This property endows \codename to deploy a flexible protection scheme $T_p$, namely to protect logs in memory at an adjustable frequency of $T_p$.
Thus, \codename bypasses the need for the costly memory copy in EL3 in a FIFO manner.
In particular, \codename registers a hardware timer inside the CPU core after initializing its HD.
We believe such a timer is widely available as built-in hardware in modern CPUs~\cite{wang2022rttee}.
The timer routinely prompts an interrupt to enforce the protection (\circleblack{\Aa{3}{b}}) at a frequency of $T_p$.
In principle, a more frequent $T_p$ shrinks the protection time window, providing better security assurance, but also increases system overhead due to more system response costs.
In practice, we find a $T_p$ of 1 ms to strike a balance between efficiency and security assurance, which we evaluate in (\cref{sec:sec_evaluation}) and (\cref{sec:performance_evaluation}).

\noindent\textbf{Buffer pool management.}
Recall that \codename maintains a \textit{current} buffer (\cref{sec:observability_generation}) to stage logs.
When the protection scheme is enforced, \codename directs the SM to protect this buffer using the primitive abstraction \hwno{5} in~\cref{tab:hw_abstraction}, which modifies the \Aa{GPT}{NS}'s buffer permission as inaccessible to the OS (\circlered{2\scriptsize{a}}).
Before doing so, the trusted gateway verifies the validity of the current buffer's metadata, such as its physical address and size.
After protecting the current buffer, a new one is retrieved from the pool to serve as the \textit{current} (\circleblack{3\scriptsize{c}}).

\noindent\textbf{Guaranteed protection scheme enforcement.}
Given the protection frequency of $T_p$, the maximal protection latency for each log after generation is $T_p + \epsilon$.
Here, the extra $\epsilon$ is due to SM response overhead (e.g., secure monitor invocation, context switch, and primitive configuration in \circlered{\Aa{2}{a}}).
Moreover, an attacker can even triggers a lot of adversarial interrupts ~\cite{lee2021exprace} to disturb the protection scheme and enlarge the protection time window.
To enforce $T_p$ and keep this $\epsilon$ nominal, \codename ensures its protection scheme is peformed in an atomic context.
During its enforcement, the CPU is inside a non-preemptible state with all interrupts disabled.

==> tex/motivation-old-2.tex <==
\section{Background}


\subsection{System Observability}
\label{subsec:system_observability}

% System observability is thesystem_model capability achieved by collecting system runtime states at different layers as {\em logs}.\adil{repetitive with intro's first sentence}
%
Observability logs provide visibility into enterprise computer's {\em security posture}, and are captured by Security Information and Event Management (SIEM) from the industry~\cite{vmware_survey,SIEM-logs} and academia~\cite{yu2021alchemist,datta2022alastor}.
% 
Based on standard security practices~\cite{obs_sec}, we consider three main sources (or layers) of logs: (a) {\em application logs} for program execution semantics~\cite{hassan2020omegalog}, (b) {\em audit logs} for OS system call events~\cite{king2003backtracking}, and (c) {\em network logs} for network traffic surveillance~\cite{datta2022alastor}.

%
As common in both widely-deployed available software~\cite{ebpf, auditd, tracee} and the literature~\cite{pasquier2017camflow,lim2021provbpf,thomas2018camquery}, there are three main components in a conventional observability log collection stack~(\cref{subfig:overview-native}). 
%

First, {\em an in-kernel log generator} is to capture system events and generate logs.
%
Given the kernel's privileged ability to oversee and control the entire system~\cite{ebpf}, events among different layers can be captured by various {\em probes} (\eg Linux Kprobe and Tracepoint).
%
Second, {\em a userspace log daemon} is to manage logs.
%
Once captured, logs are transmitted from the kernel to the user daemon to support log management tasks (\eg filter, query, and remote retrieval).
%
Last, {\em a storage device} finally keeps all logs persistent locally. 

% \begin{enumerate}[leftmargin=*,label=\textbullet]
%     \item
%     {\em An in-kernel log generator} to capture events and generate logs.
%     %
%     Given the kernel's privileged ability to oversee and control the entire system~\cite{ebpf}, 
%     events among different layers can be captured by various {\em probes} (\eg Linux Kprobe and Tracepoint).
%     \item
%     {\em A userspace log daemon} to manage logs.
%     %
%     Once captured, logs are transmitted from the kernel to the user daemon to support log management tasks (\eg filter, query, and remote retrieval).
%     \item 
%     {\em A storage device} finally keeps all logs persistent. 
% \end{enumerate}
%

% \AD{There's too many bullet lists in the first two pages. You may inline the above list, since it's less important.}

% Once logs are collected at the host enterprise machine, the IT administrators are responsible for maintaining them. 
% %
% To do so, the administrators will periodically retrieve logs from the enterprise computer and send them to their servers through the log daemon.
% 

% \subsection{CPU Privilege Levels}
% \label{sec:arm_background}
% %
% Modern CPU processors have different execution privilege levels (\eg ARM exception levels or x86 protection rings), including {\em applications}, {\em OS}, {\em hypervisor}, and the {\em management mode} (so-called ARM's monitor mode or x86 system management mode) ordered by their hardware privileges from low to high.


% %
% % ARM CPUs have four exception levels: applications (EL0), the OS (EL1), the hypervisor (EL2), and system management mode (SMM, EL3).
% %
% Higher privilege levels can interpose lower levels (\eg manipulate their memory and system registers).
% %
% In this regard, management mode is at the highest level (ARM exception level EL3 or x86 ring -2). 
% %
% It controls fundamental system resources (\eg interrupt and power management) and provides secure firmware for the system, such as trusted boot primitives (\eg for UEFI secure boot~\cite{Richardson2013UefiSB}) and kernel context interposition (\eg for TrustZone secure OS~\cite{cerdeira2020tzsok}).
% %
% The OS can issue a synchronous exception (ARM Secure Monitor Call SMC or Intel System Management Interrupt SMI) to trap into and synchronize the management mode for runtime services~\cite{atf}.

% \chuqi{TBD: do we need this section?}


% \PP{Granule protection table (GPT).}
% %
% GPT is an in-memory (page-table-like) infrastructure introduced by Realm Management Extension (RME)~\cite{rme-extension} of Confidential Computing Architecture (CCA).
% %
% CCA introduces four CPU {\em security states}: normal, secure (for TZ secure world), realm (for CCA's confidential VMs~\cite{cca}), and root (exclusively for EL3).
% %
% It allows dynamically configuring a physical memory granule's (page-level) accessible states ({\em \eg normal, secure, realm, root, all, or none}).
% %
% Each last-level GPT entry controls up to sixteen physical pages' accessible CPU states~\cite{rme-extension-website}.
% %
% During the page table walk, RME hardware enforces MMU to perform a granule protection check (GPC) and check the target page's access permission.
% %
% The GPT's program interface (\ie control register and table edit) is exclusive to SMM.


\subsection{Threat Model and Assumptions}
\label{subsec:threat_model}

Like recent work in log protection~\cite{varun2023omnilog,ahmad2022hardlog,riccardo2020kennylogging,paccagnella2020custos}, we assume the enterprise host system is initially benign, but a \textit{non-privileged remote adversary} starts to attack it at time $t_s$.
%
The adversary exploits software and kernel vulnerabilities in the host system to
(a) circumvent the common defenses~(\eg ASLR, DEP, and stack canaries) and 
% (b) escalate the privilege to the root at time $t_c$.
(b) compromise the full system at time $t_c$.
% \AD{There's a difference between privilege escalation and kernel compromise. Do you mean compromise?} 
%
Being aware of mechanisms of the system observability, the adversary attempts to tamper with the logs in kernel memory or on storage, striving to hide the attack footprints (\ie logs between $t_s$ and $t_c$)~\cite{mitrelinuxlogs,mitrewindowslogs}.

%
Before $t_c$, the observability log generator is honestly deployed inside the OS to capture logs.
Post OS compromise (after $t_c$), adversaries gain full system control and then prevent the log capture (\eg they can simply halt the in-kernel log generator).
% 
Hence, logs after $t_c$ are {\em worthless} for forensic analysis~\cite{ahmad2022hardlog,varun2023omnilog}.
%

{\bf \em Assumptions.}
%
%
We make standard assumptions that enterprise parties (OS vendors and administrators), computer hardware, and firmware (\eg UEFI) are trustworthy.
%
In addition, cryptographic protocols and key management schemes work correctly. 
%
Moreover, we assume the secure boot protocol is trustworthy for authenticating system configurations, ensuring the system is always benign initially.
%
% Finally, if (and only if) virtual machines are supported on the host machine and S2PT is used for permission switching, we assume that the security monitor interposes S2PT interfaces (see discussion in \cref{sec:discussion}).
We finally assume only {\em forensics-critical} logs (specified in \cref{subsec:system_observability}) should be protected, as they are the primary targets of the adversaries.
%
System display messages, such as {\em dmesg}~\cite{dmesg}, are out of scope.
%
Regardless, the administrator can configure the observability generator to specify what logs to be protected (\cref{subsec:design_realtime_deadline}).


% We make standard assumptions that IT administrators, computer hardware, and firmware (\eg UEFI, BIOS) are trustworthy.
% %
% In addition, we assume that cryptographic protocols and key management schemes are as expected. 
% %
% Finally, we assume that the secure boot protocol is trustworthy to authenticate system configurations and key provisions, ensuring the system is always benign initially.

\begin{figure*}
    \centering
    \captionsetup[subfloat]{justification=centering}
    \subfloat[Conventional (observability) \\ logging systems~\cite{ebpf,tracee,auditd}.]{
        \begin{minipage}[t]{0.22\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/overview-native.pdf}
            \vspace{-0.3cm}
            % \subcaption{{\footnotesize (a)}}
            \label{subfig:overview-native}
        \end{minipage}
    }
    \subfloat[Logging systems with in-memory \\ trusted kernels~\cite{varun2023omnilog,shepherd2017emlog}.]{
        \begin{minipage}[t]{0.23\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/overview-omnilog.pdf}
            \vspace{-0.3cm}
            % \subcaption{{\footnotesize (c)}}
            \label{subfig:overview-omnilog}
        \end{minipage}
    }
    \subfloat[Logging systems with external \\ tamper-proof audit devices~\cite{ahmad2022hardlog,sekar2024eaudit}.]{
        \begin{minipage}[t]{0.23\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/overview-hardlog.pdf}
            \vspace{-0.3cm}
            % \subcaption{{\footnotesize (b)}}
            \label{subfig:overview-hardlog}
        \end{minipage}
    }
    \subfloat[\codename \\ (this work).]{
        \begin{minipage}[t]{0.23\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/overview-hitchhiker.pdf}
            \vspace{-0.3cm}
            % \subcaption{{\footnotesize (d)}}
            \label{subfig:overview-hhk}
        \end{minipage}
    }
    \caption{Overviews of (a) conventional observability systems and (b-d) observability protection systems (\boxhd\ : trusted components).}
    \label{fig:overview}
    \vspace{-0.2cm}
\end{figure*}
% \adil{ideas: 
%     (a) Consider showing that a log with OmniLog is generated at kernel, copied to monitor, and then copied to daemon using a background thread~(2 copies). 
%     (b) Consider showing the two OmniLog designs separately (not sure), 
%     (c) somehow you want to show the extra interfaces (attack surfaces) of OmniLog (e.g., Hypervisor interface, OPTEE interface)}


\section{Motivation}
\label{sec:motivation}

\subsection{Observability Protection}
\label{subsec:existing_solutions}
%
An observability protection system is deployed to shield both log integrity and availability. 
% 
% This section describes (a) the high-level aspects required for observability protection, and (b) the state-of-the-art approaches to protect logs.
% 
% 
In general, there are two main aspects to the observability log (from any sources)
% (or any kind of log generated from anywhere in the system) 
protection.
% needed to provide integrity and availability of logs with the following aspects.

%
First, a {\em log protection scheme} determines {when to shield logs} from the untrusted OS after their generation. 
%
This can be {\em synchronous} or {\em asynchronous}. 
% 
In the former case, each log is secured immediately after generation (\ie blocking a syscall until its corresponding log entry is protected). 
% 
In the latter case, logs are batched in the OS memory after generation and periodically protected.
%

%
Second, a {\em secure log environment} is required to {safely hold and manage logs} in a persistent manner.
% 
This environment is either a combination of a secure in-memory environment and a protected disk, or only a secure disk (\eg remote storage).
%
% \begin{enumerate}[leftmargin=*,label=\textbullet]
%     \item
%     A {\em log protection scheme} determines {when to shield logs} from the untrusted OS after their generation. 
%     %
%     This can be {\em synchronous} or {\em asynchronous}. 
%     % 
%     In the former case, each log is secured immediately after generation (\ie blocking a syscall until its corresponding log entry is protected). 
%     % 
%     In the latter case, logs are batched in the OS memory after generation and periodically protected.
    
%     \item 
%     A {\em secure log environment} is required to {safely hold and manage logs} in a persistent manner.
%     % 
%     This environment is either a combination of a secure in-memory environment and a protected disk, or only a secure disk (\eg remote storage).
% \end{enumerate}

\PP{Existing solutions.}
In terms of synchronous log protection, OmniLog~\cite{varun2023omnilog} is the state-of-the-art system~(\cref{subfig:overview-omnilog}). 
% 
It blocks the system and synchronizes the log by copying it to a privileged host system layer, a so-called {\em security monitor}.
% 
The high I/O latency makes it impractical to directly store each log entry synchronously to disk. 
% 
% Hence, OmniLog constructs an in-memory secure environment using a higher system layer at a privileged CPU level than the OS~(\eg the x86 hypervisor and ARM TrustZone).
Hence, OmniLog constructs an in-memory secure environment based on its security monitor~(\ie the hypervisor and ARM TrustZone).
%
Logs are kept in this environment before being eventually written to a protected disk.
% Once a log entry is generated, it blocks the OS and copies the log to this in-memory secure environment~(\eg a trusted virtual machine), which later dumps it onto protected storage.
%
Other solutions~\cite{dunlap2002revirt,shepherd2017emlog} follow a similar approach to building a secure environment.
%

%
Alternatively, solutions~\cite{ahmad2022hardlog,sekar2024eaudit} asynchronously protect logs by using {\em write-once-read-many} (WORM) or custom device.
%(\ie the secure environment is the disk).
% 
Due to inherent I/O latencies, such systems are forced to use asynchronous protection.
% 
% Alternatively, asynchronous protection is widely adopted when opting for external secure environments rather than in host memory, for the performance reason.
%
In this regard, HardLog~\cite{ahmad2022hardlog}~(\cref{subfig:overview-hardlog}) is the state-of-the-art. 
%
It batches logs in OS memory and periodically sends them to a custom audit device, which stores logs from the host and also supports retrieval tasks.
% 
Besides that, some asynchronous systems also batch and transmit logs to a network storage server~\cite{anjo2015guardat,robert2018pesos}.
% \adil{fix order, your figures have async coming first.}

% \adil{I'm not sure the above is the best place to talk about these systems. Could we merge with section 3?}
% \chuqi{check}

% \adil{needs top-down.}


\subsection{Limitations of Current Protection Solutions}
\label{subsec:limitations_of_existing_protection_solutions}

% Prior solutions have the following limitations: (L1) synchronous protection solutions incur {\em significant slowdown for log-intensive real-world programs}, 
% % 
% (L2) asynchronous protection solutions provide {\em large attack windows that lead to tampering}, 
% and 
% (L3) in-memory protection solutions {\em keep logs in low assurance environments that can be compromised}.
%
% We further analyze them in the following paragraphs.
%

%
\PP{L1: Slow synchronous protection in log intensive scenarios.}
%
Modern computers can produce lots of observability logs when running realistic I/O-intensive real-world programs.
%
Under such scenarios, synchronously protecting every produced log, even in memory, imposes a notable slowdown.
% 


% 
To concretely show the slowdown, we synchronously protected logs produced by three high-performance programs: web server ({\em Nginx}), in-memory key-value store ({\em Redis}), and on-disk relational database ({\em MySQL}).
%
% \sout{Our host server is an ARM-Juno R2 device with a dual-core A72 and a quad-core A53 alongside 8GB memory, and 1TB SSD.}
%
Programs are tested with default configurations and benchmark settings of {\em apachebench}~\cite{ab}, {\em memtier\_bench}~\cite{memtier}, and {\em sysbench}~\cite{sysbench}, respectively.
We employed the synchronous protection of OmniLog~\cite{varun2023omnilog}~(detailed setup can be found in~\cref{sec:performance_evaluation}).
% 

%   
% \adil{"This" is in the last paragraph. Don't use "this for cross-paragraph aspects".}
\cref{tab:obs_throughput} illustrates the performance impact incurred by OmniLog and the conventional observability generator (Native-OBS), which stores logs within the kernel's memory, against native execution.
% 
We observe that OmniLog's synchronous protection incurs $0.9-7.2\times$ more overhead than Native-OBS.
%
Due to the high throughput of observability logs, synchronous protection for each log requires frequent system interruption, involving context switches to the privileged layer (\eg changing the protection ring in x86 or the exception level in ARM), and copying the log to the protected memory inside a privileged layer, which is time-consuming.
%
% In~\cref{subsec:overview_inmemory_observability_protection} and~\cref{tab:prot_primitives}, we discuss how privileged memory copy can affect system performance significantly.\chuqic{We may not want to highlight the memcpy's overhead}

\begin{table}[t]
    %\vspace{-0.3cm}
    \centering
    \caption{Multi-layer observability log throughput, log capture overhead, and synchronous log protection~\cite{varun2023omnilog} overhead.
    \textbf{Audit Log}: system call logs~\cite{auditd};
    \textbf{App. Log}: application logs~\cite{hassan2020omegalog};
    \textbf{Net. Log}: network event logs~\cite{ujcich2021causal}.
    % \adil{Font is too small. Reduce space between columns to enlarge.}\chuqi{fixed}
    }
    \vspace{-0.2cm}
    \label{tab:obs_throughput}
    \setlength{\aboverulesep}{0.05pt}
    \setlength{\belowrulesep}{0.05pt}
    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.0}
    \begin{adjustbox}{width=1\linewidth}
    \begin{threeparttable}
    \begin{tabular}{@{}lcccc|cc@{}}
    \toprule
    \multirow{2}{*}{\textbf{Program}}                     & \multicolumn{4}{c|}{\textbf{\#Multi-layer Observability Throughput}\tnote{\textbf{1}}} & \multicolumn{2}{c}{\textbf{Overhead (\%)}} \\ \cmidrule(l{\dimexpr0.1cm+1pt} r{\dimexpr0.1cm+1pt}){2-5}\cmidrule(l{\dimexpr0.1cm+1pt} r{\dimexpr0.1cm+1pt}){6-7} 
    \multicolumn{1}{c}{}                                  & \textbf{Audit Log}  & \textbf{App. Log}  & \textbf{Net. Log} & \textbf{Total}\tnote{\textbf{2}} & \textbf{Native-OBS}  & \textbf{\omnilog}  \\ \midrule
    \textbf{Nginx}                                        & 53,038              & 25,144                    & 594                  & 78,776         & 4.2\%             & \textbf{15.4\%}      \\
    \textbf{Redis}                                        & 40,857              & 152                       & 37,528               & 78,537         & 6.4\%             & \textbf{52.6\%}      \\
    \textbf{MySQL}                                        & 76,228              & 5,151                     & 20,583               & 101,962        & 13.8\%             & \textbf{27\%}      \\ \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \item[\textbf{1}]
        {Throughput (logs/second) is counted by the conventional log generator (\textbf{Native-OBS}; \cref{sec:impl}) under the real-world workload detailed in~\cref{tab:workloads} (\cref{subsec:performance_evaluation}).}
        \vspace{0.05cm}
        \item[\textbf{2}]
        {Each log entry is around 256 bytes on average size.}
    \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
    % \vspace{-0.5cm}
\end{table}

\PP{L2: Insecure {I/O-based} asynchronous protection window.} 
%
Current asynchronous protection systems~\cite{ahmad2022hardlog,sekar2024eaudit,riccardo2020kennylogging,paccagnella2020custos} expose a long time window before logs are protected to remote or local {\em tamper-proof} storage through slow I/O operations.
%
% This enables adversaries to compromise logs in memory within the protection window.
% 
For instance, the state-of-the-art HardLog~\cite{ahmad2022hardlog}, provides a lengthy \textms{15} delay.
%
% This window is due to the I/O latency between the batching of logs in host kernel memory and their transmission to an external secure environment, \ie a secure USB drive.
%
Unfortunately, adversaries can exploit kernel vulnerabilities and obtain root access within very few syscalls~\cite{overlayfs-exp}, each of which only requires thousands of cycles, and tamper with in-kernel logs.
%

% %
% To better illustrate the tampering problem, we executed PoC exploits for ten kernel common vulnerabilities and exposures (CVEs) in the past three years to tamper with logs.
% %
% CVEs are selected from well-known security assessment forums (\eg\ {\em Seclist, Openwall}) with high Common Vulnerability Scoring System (CVSS)~\cite{cvss} scores.
% %
% Also, they are collected from two major categories~\cite{chen2011linuxkernel}: (i) semantic bugs like improper permissions or security checks, and (ii) memory corruptions (\eg stack or heap-related temporal and spatial corruptions).
% %
% As typical in tampering research, our experiments assumed the adversary had already gained an unprivileged foothold in the system.
% %
% We ran automated scripts that (a) executed the PoC exploits to gain root and (b) loaded a kernel module to delete the log buffer.
% % 
% Each attack is performed ten times.
% %
% \cref{tab:top5_attacks} highlighted the top-5 fastest attacks (detailed studies and discussions are in~\cref{subsec:case_study}).

% \adil{Start with something like: "Our experiments show that common vulnerabilities can tamper logs within a 15ms window."}\chuqi{fixed}

To understand the tampering problem, consider the DirtyPipe~\cite{dirtypipe} attack due to improper preservation of permissions.
%
Given a flaw of a simple improper \textcode{PIPE\_BUF\_FLAG\_CAN\_MERGE} flag in kernel, the vulnerability offers adversaries the capability to quickly rewrite arbitrary files (\eg \textcode{/etc/passwd}) to escalate privileges.
% 
% We used automated scripts to run its PoC exploit and load a kernel module to delete the kernel log buffer.
We reproduced its PoC exploit to load a kernel module to delete the logs.
% 
We found that it took within around $12ms$ (detailed case study in~\cref{subsec:case_study}), resulting in scenarios where {\em all} attack traces were lost in \textms{15} windows.
% 
This exploit arises from a semantic bug. Unlike common memory corruption vulnerabilities, exploiting such bugs does not require slow object manipulation or heap spraying~\cite{lin2022dirtycred}, making them brutal and ``efficient'' for adversaries.
% 

%
Please note that this simple example does not show that a \textms{15} protection delay is insufficient to prevent tampering in the majority of kernel attacks.
% 
However, it does indicate that {\em PoC exploits (which are not designed to be fast) for common attacks can allow log tampering within a \textms{15} window}, highlighting the need to shrink the protection window to significantly raise the bar of attacks.


\begin{table}[t]
  \caption{
  The percentage of discovered vulnerabilities in general-purpose system components and interfaces~\cite{chen2023security,cerdeira2022rezone,cerdeira2020tzsok,Shi2017DeconstructingXen} used by prior in-memory log protection systems.
  }
  \vspace{-0.2cm}
  \label{tab:general_purpose_attack_surface}
  \setlength{\tabcolsep}{3pt}
  \setlength{\aboverulesep}{-0.03pt}
  \setlength{\belowrulesep}{-0.03pt}
  \begin{adjustbox}{width=\columnwidth, center}
    
    \begin{tabular}{|cccc|ccc|}
    \hline
    \multicolumn{4}{|c|}{\textbf{Hypervisor (\ie VMM)}} & \multicolumn{3}{c|}{\textbf{TrustZone}} \\ \hline
    \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}VM memory\\ manage.\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}CPU\\ virtualiz.\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Code\\ emulation\end{tabular}}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Device\\ I/O\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Trusted\\ Apps.\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}TZ \\ kernel\end{tabular}}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}TZ memory\\ manage.\end{tabular}}} \\
    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
    \multicolumn{1}{|c|}{25.7\%} & \multicolumn{1}{c|}{21.5\%} & \multicolumn{1}{c|}{13.2\%} & 9\% & \multicolumn{1}{c|}{33.2\%} & \multicolumn{1}{c|}{27.8\%} & 17.1\% \\ \hline
    \end{tabular}
  \end{adjustbox}
  % \vspace{-0.5cm}
\end{table}

\PPn{L3: Low assurance secure environments.}
%
Prior work~\cite{varun2023omnilog,shepherd2017emlog,dunlap2002revirt} adopts virtual machine manager (VMM) or TrustZone (TZ) to protect logs in memory.
%
However, their bloated interfaces enlarge the vulnerabilities within the secure environment.

%
% Logs are kept within the trusted kernels of virtual machines or the TZ secure OS)~\cite{varun2023omnilog,dunlap2002revirt,shepherd2017emlog}.
Logs are kept and managed within trusted kernels, such as feature-rich virtual machines or the TZ secure kernels (\eg OP-TEE~\cite{optee}). 
%
Supporting such environments involves complex interfaces, such as CPU virtualization, code emulation, and TZ management.
%
Unfortunately, those full-fledged general-purpose interfaces enlarge the vulnerabilities~\cite{cerdeira2022rezone,brasser2019sanctuary,Shi2017DeconstructingXen,zhou2023coreslicing} on the system.
%
For instance, a single vulnerability in CPU (interrupt) virtualization leads to host kernel arbitrary code execution~\cite{cve-2018-16882}.
%

% The bloated interfaces of the full-fledged virtual machine manager (VMM) and TrustZone (TZ) undermine the assurance of the secure log environment.

% Logs are kept within the trusted kernels of VMM or TZ (under a virtual machine or the TZ secure OS)~\cite{varun2023omnilog,dunlap2002revirt,shepherd2017emlog}.

% If general-purpose clients (feature-rich VMs or trusted applications) have to be supported, 

\cref{tab:general_purpose_attack_surface} then concretely concludes the discovered vulnerabilities within general VMM and TZ interfaces.
%
% In principle, all their brought interfaces are redundant for supporting log management.
%
Considering the severe vulnerabilities inside VMMs, 72.07\% and 80.81\% of the common vulnerabilities and exposures (CVEs) in KVM~\cite{qumranet2007kvm} and Xen~\cite{xen} can lead to host exploitations, respectively~\cite{chen2023security}.
%
Meanwhile, more than 65\% of CVEs in TZ kernel-supported systems~\cite{cerdeira2020tzsok} have severe ($\ge 7$) common vulnerability scoring system (CVSS~\cite{cvss}) scores.


%
% Prior research~\cite{varun2023omnilog,dunlap2002revirt,shepherd2017emlog} that protect and manage logs in memory either rely on (a) full-fledged virtual machine manager (VMM) or (b) ARM TrustZone (TZ) secure world alongside the trusted kernels.
% %
% Logs are held in a virtual machine or TZ kernels like OP-TEE~\cite{optee} as secure environments.
%
% These approaches cannot provide high assurance: they require a large TCB and expose a significant attack surface (\cref{subsec:overview_secure_environment}).
%
% These approaches are complex and bloated for logging, undermining the assurance of the secure environment.
% \AD{Rewrite this paragraph and start with the takeaway first. Currently, this paragraph is hard to understand and all over the place.}

%
% General-purpose solutions like VMM and TZ include extensive redundant functionalities from the host system components.
% To further understand the attack surface, we analyze the interfaces of components (\eg VMM, TZ) and their CVEs reported by recent studies and source code~\cite{cerdeira2020tzsok,agache2020firecracker, chen2023security}.
% General-purpose components (VMMs and TZ) have large attack surfaces~\cite{cerdeira2022rezone,brasser2019sanctuary,Shi2017DeconstructingXen,zhou2023coreslicing}, by exposing intensive interfaces to their clients. 
%
% \AD{You need to expand more here. The reviewer asked for a more nuanced explanation, this section is not doing enough.}

% Considering the severe vulnerabilities inside VMMs, 72.07\% and 80.81\% of the total CVEs in KVM~\cite{qumranet2007kvm} (111 in total) and Xen~\cite{xen} (370 in total) during fourteen years can lead to host-kernel exploitations, respectively~\cite{chen2023security}.
% %
% Meanwhile, more than 120 CVEs have been revealed in different TZ kernel-supported systems during six years~\cite{cerdeira2020tzsok}, while 65\% of them have severe ($\ge 7$) CVSS scores.
%
% \cref{tab:general_purpose_attack_surface} further concludes the majority of attack targets within the general hypervisor and TZ interfaces.\AD{Give the reviewer details. Don't expect them to read the table. Also, offer an intuitive reason as to why this may be the case.}
% %
% Relying on these heavy and full-fledged components' support for log protection unnecessarily increases both complexity and security risks~\cite{hof2022blackbox}.

%
% \AD{Start with the "large" attack surface first. Then, as proof that this attack surface is "bad", cite the CVEs.}\chuqi{check}

% \AD{"bloating general-purpose" is a weird term, and also seems unnecessary. You don't need to explain everything within the heading, just the key aspect.}\chuqi{check}

% \AD{Can we also say XYZ \# of vulnerabilities have been found in TZ/HV here? We may move our analysis from 7.4 to here if it makes sense.}\chuqi{check}



% However, those general-purpose interfaces are non-necessary for logging tasks.
% %
% Both CPU virtualization, VM management, and code emulation are not desired by log management tasks, yet should be supported by VMM~\cite{xen,qumranet2007kvm} for an in-VM secure environment.\AD{you don't need to say this here. Here you only need to convince reviewers that using HV/TZ is a bad idea.}
% %
% % Even a host-based virtualization\AD{incomplete?} 
% %
% Similarly, TZ kernels support executing regular rich trusted applications, TAs~\cite{pinto2019demystifying}), exposing large interfaces to both native OS and TAs (\eg at least four daemons in an Android OS have privileged access to TZ kernel interfaces~\cite{cerdeira2020tzsok}).
% %
% As a result, holding the secure log environment into TZ undesirably inherits TZ's attack surfaces~\cite{cerdeira2022rezone,brasser2019sanctuary}, which are not necessarily required for log management tasks.\AD{same comment as above applies here.}
%

% \adil{What does it mean for the percentage to be "attack surfaces"? Do you mean that x\% vulnerabilities are in such components? If yes, please be precise.}\chuqi{changed to the nestedXen's term ``attack targets''}

% Both hypervisor ({\em aka} Virtual Machine Manager, VMM) and TZ are general-purpose layers within enterprise settings that expose complex interfaces to their clients.
% 
% \chuqic{Specifically}, virtualizing even a single OS (host-based virtualization) requires virtualization software~\cite{bareflank,jailhouse} to handle complex hardware functionality (\eg second-level translation) and provide \sout{several} \chuqic{a large amount of} services to the OS (\eg control register emulation, interrupt redirection). 
% 
% If additional guest VMs (\eg for log management or general client) are supported, a larger TCB is needed~\cite{xen,qumranet2007kvm} to support services like memory management and device emulation. 
% %
% Similarly, TZ supports the entire secure world (\eg KNOX~\cite{knox} adopts TZ as runtime support for executing regular rich trusted applications, TAs~\cite{pinto2019demystifying}).
% %
% A TZ kernel, therefore, exposes large interfaces to both the native OS (\eg at least four daemons in an Android OS have privileged access to TZ kernel interfaces \sout{to access TAs}~\cite{cerdeira2020tzsok}) and to support OS services feature-rich TAs.
% %
% A vulnerability that is common in such large components can be exploited by an attacker~\cite{cerdeira2020tzsok,cerdeira2022rezone,chen2023security}.
%
% We provide detailed TCB and attack surface discussions in~\cref{subsec:overview_secure_environment} and~\cref{subsec:tcb_evaluation}.

% \adil{add rebuttal stuff, do CVE study}
% \adil{I feel like you need to rethink L3 from the ground-up. The reviewers were not convinced.}

% \adil{For above: what about host-based virtualization that does not use a hypervisor, like what OmniLog says you should use?}
% \chuqi{Let me think then... Seems still a question about a micro VMM + micro VM?}

% %
% Concretely, the popular combination of Linux Kernel Virtual Machine (KVM) and QEMU (used by~\cite{varun2023omnilog}) requires 1.5 million lines of code with up to 270 unique syscalls~\cite{agache2020firecracker}.
% %
% Even a TrustZone kernel like OP-TEE~\cite{optee} is concerned to be debloated, 
% it still contains over 300 thousand lines of code with 70 syscalls.
% %
% Therefore, even though their attack surfaces are smaller than traditional OSs, they are still considerably large by sharing interfaces and attack vectors with their clients~\cite{cerdeira2022rezone,cerdeira2020tzsok,agache2020firecracker}.
% % 
% \adil{I don't understand this. Why is the OPTEE syscall interface an attack vector? Are you assuming the TA is compromised by OS, and then launches an attack against OPTEE OS?}\chuqi{Yes, a TA can be easily compromised?~\cite{cerdeira2022rezone} Also I-02 in~\cite{cerdeira2020tzsok}}


%
% \adil{weak language, be more direct (e.g., a bug/vulnerability which is common in such large kernels can be exploited by an attacker.)}\chuqi{fixed. rewrote this subsection}

% This raises concerns about the overall security assurance of the log protection environment and makes it hard for verification.
%
% For example, simply reusing the drivers\adil{comes out of nowhere. You're talking about kernels above.} from a commodity trusted guest kernel for log persistence, as the practice of~\cite{varun2023omnilog}, inherents its complex and buggy driver TCB~\cite{wang2022rttee,guo2022driverlet}.
%
% As such, employing a trusted kernel brings along all its extensive and potentially vulnerable codebase.


% \subsection{\codename Goals and Principles}
% \label{subsec:research_goal}

% % Given an untrusted OS, the adversary can compromise the entire observability software 
% % stack, thereby eradicating all historical logs as a forensics countermeasure.
% % %
% % Indeed, log removal is a common tactic in APT campaigns and malware~\cite {mitrewindowslogs,mitrelinuxlogs,hermeticwiper,killdisk,dazzlespy}, serving as an attack indicator elimination method.
% %

% % This paper's goal is to \textit{design a secure system observability infrastructure, \codename, to provide integrity and availability of observability logs generated prior to OS compromise, and securely manage the logs} with:
% \adil{Designing a system is not your goal. Solving a problem is your goal. Your system is a consequence of your goal.}
% \adil{Configurable performance/security (trade-off)? Something about {\em configurability} would be nice here.}
% \chuqi{revise}
% \chuqi{FAILE to make a crisp section :( Also FAILED in 4.3}

% Given existing protection systems and their drawbacks, \codename aims at (a) residing in a sweet spot for optimized performance and security, and (b) building a high-assurance secure environment to protect the integrity and availability of system observability.
% %

% In particular, a {\em real-time configurable log protection deadline} should be enforced.
% %
% Each log, after generation, should be protected {\em in host memory} within a very narrowly defined deadline.
% %
% This obviates I/O latency to ensure a tiny protection window, raising an unrealistically challenging window for adversaries to compromise logs.
% %


% In addition, a secure environment {\em dedicated to observability protection and management} should be maintained.
% %
% It should not rely on large general-purpose layers (\eg VMM or TZ), reducing shared attack surfaces with other system components.
% %
% Furthermore, functions crucial to protect log integrity and availability should be kept debloated and tiny in this secure environment (TCB).
% %
% Non-critical log management (\eg log daemon execution) support should be securely delegated to the OS rather than be included in TCB.
% %
% This constrains TCB, preventing including large commodity trusted kernel from exploding it.

% \PP{G1: Balanced performance and security}
% %
% We aim to reside in a sweet spot between
% %
% (a) runtime overhead, ensuring the practicality and scalability of the system; and 
% %
% (b) protection latency, enabling logs to be efficiently protected after their generation, thus preventing log tampering attacks.

% \PP{G2: High-assurance secure log environment.}
% %
% Our goal is to maintain a protection system dedicated to observability logs with minimal TCB and attack surface.
% %
% It is crucial to limit the common attack surface shard with other system software components.

% \PP{G3: Deployable and easy to maintain.}
% %
% The burden on system deployment is to be reduced as much as possible.
% %
% Thus, the legacy observability software stack should be minimally extended, avoiding largely modifying existing components or involving huge extra components and codebase.
% % 
% \adil{Not easy-to-understand this third one, since it's not a limitation of prior work (atleast you did not mention it). I'd say mention this within the design itself, instead of mentioning here.}
% \chuqi{Can we just put this point upfront here (like Shuffler) to give reviewers a better hint?}\adil{I don't love that idea, since it'll confuse reviewers. Let's leave it for now.}



==> tex/observability_generation.tex <==
\section{Observability Generation}
\label{sec:observability_generation}

eBPF offers a non-intrusive way to run subprograms in-kernel for runtime observability collection.
Those programs can be attached to various events (e.g., tracepoints, kprobes, and uprobes) and access kernel data structures within event contexts.

\chuqi{should move this paragraph to implementation?}

\codename leverages eBPF to build its observability generator.
During runtime, the \codename injects BPF programs to all 436 system calls and socket-related events to support audit and network logging.
To collect application logs, \codename extracts kernel data from write-related syscalls.
For instance, by extracting \texttt{file} structure from syscall \texttt{fd} parameter in runtime task context, \codename matches predefined paths (e.g., /var/log/a.log) to determine application logs.
Further, \codename extracts the log content from the userspace buffer parameter.

To unify multiple layer log collection (\circleblack{1}--\circleblack{2}) into \codename's protection pipeline, \codename reserves a kernel \textit{buffer pool} for the generator.
This pool is statically allocated during secure boot in a reserved physical region with a fixed address range (M{\scriptsize{BUFPOOL}} in~\cref{fig:workflow}).
In particular, \codename maintains a \textit{current} buffer for the generator to write all logs (\circleblack{3\scriptsize{a}}).
To do so, \codename extends eBPF helper interfaces with a new one named \texttt{bpf\_write\_current\_buf}.
Extending BPF helpers is a common practice in existing works~\cite{lim2021provbpf}.
We believe the modification is simple (requires less than 50 lines of kernel code change for BPF verifier support) and will not expand \codename's attack surface.
% \adil{Only talk about interesting things here like how HHK collects logs from different sources in one place efficiently.}


==> tex/overview-old-2.tex <==
\section{\codename Overview}
\label{sec:design_overview}

% Inspired by limitations of the existing work (\cref{subsec:limitations_of_existing_protection_solutions}), this section describes two key design principles of our system, \codename.
% % 
% Given the rising use of ARM-based computers in enterprises and cloud computing, we use ARM as the reference architecture.
% % , where the related features are described in~\cref{sec:arm_background}.
% %
% We discuss \codename's portability to other architectures in~\cref{sec:discussion}.

% Inspired by the limitations of existing work, we propose \codename.
%
\codename is an efficient and high-assurance observability protection system.
%
\cref{subfig:overview-hhk} presents its high-level architecture.
%
%
Compared with existing solutions, two {\em key design principles} are applied.
% for efficient and secure log protection and management.
\vspace{-0.15cm}
\begin{enumerate}[leftmargin=*,label=\textbullet]
    % \item
    % TrustZone Address Space Controller (TZASC) allows access control over a contiguous memory region (at least 32KB) at the memory bus transaction level by configuring its control registers, which is introduced from TrustZone hardware features~\cite{tzc400}.    
    \item
    To overcome {\bf L1} and {\bf L2}, each generated log {\em is protected in memory within an enforced short real-time deadline} before being persisted.
    %
    Hardware permission switching is applied to further reduce overheads during log protection~(\cref{subsec:overview_inmemory_observability_protection}).
    % by swift memory permission switches~(\cref{subsec:overview_inmemory_observability_protection}), .
    %
    \item
    To overcome {\bf L3}, a dedicated, high assurance secure environment that {\em does not rely on bloated general-purpose components} is instantiated to protect logs at runtime.
    %
    {Log management tasks are securely delegated to the OS}~(\cref{subsec:overview_secure_environment}).\chuqi{principle?}
\end{enumerate}
\vspace{-0.15cm}

%
Given the rising use of ARM-based computers in enterprises and cloud computing, we use ARM as the reference architecture.
% , where the related features are described in~\cref{sec:arm_background}.
%
We discuss \codename's portability to other architectures in~\cref{sec:discussion}.


% \subsection{\textbf{Configurable Deadline-Enforced In-Memory Log Permission Switch}}
% \subsection{\textbf{Fast Configurable Log Permission Switching}} 
\subsection{\textbf{Deadline-Enforced Log Permission Switch}} 
% \subsection{\textbf{Real-Time Switch-Based Log Protection}} 
% \subsection{\textbf{Real-Time Log Permission Switching}} 
\label{subsec:overview_inmemory_observability_protection}
% \AD{check name. not sure.}

% To achieve high performance while preventing strong attackers from tampering with logs (overcoming {\bf L1} and {\bf L2}),
% 
\codename protects logs in memory within short real-time deadlines set by administrators using fast hardware permission switches.
% 

In-memory protection inherently provides tighter deadlines than I/O-based protection~\cite{ahmad2022hardlog}, which suffers from large device latencies~(\cref{subsec:limitations_of_existing_protection_solutions}) and interference from other devices.
% 
% \AD{Not a good word, rephrase}
% Straightforwardly, logs are copied from the OS to the protected memory~\cite{varun2023omnilog}.\AD{This entire sentence seems to say the same thing as the first one in the para.}
Naively, at configured deadlines, logs may be copied from the OS to the protected memory~\cite{varun2023omnilog}.
%
However, short deadlines required for security result in frequent copying.
%
This causes non-negligible protection overheads in scenarios where logs are frequently produced~(\eg up to 32\% runtime performance overhead as we show in \cref{subsec:performance_evaluation}).
% 

%
{\em Switching} log buffer permissions using hardware permission primitives can mitigate the large memory copy overhead.
%
% Intuitively, using memory permission switches to protect logs avoids the time-consuming large amount of data copy, which can improve efficiency.
% ~\cite{du2019xpc, elphinstone2013l3tol4}\AD{These cites look like the idea is already used for logs.}.  
%
% This intuition is derived by adopting zero-copy temporary permission mapping for message passing optimization~\cite{du2019xpc, elphinstone2013l3tol4}.
%
To illustrate this, \cref{tab:prot_primitives} compares copying different sizes of log buffers to a privileged monitor layer (ARM's management mode or EL3~\cite{arm-manual} as used by prior work~\cite{varun2023omnilog,shepherd2017emlog}), against protecting them by hardware memory permission primitives\footnote{
TrustZone Address Space Controller (TZASC~\cite{tzc400}) is an alternative primitive.
%
Its limited regions and static set up~\cite{li2021twinvisor} lack flexibility.
% \AD{Isn't the main problem it being static?}.
%
Thus, we discuss and implement \codename via S2PT and GPT. 
%
% Regardless, TZASC is also able to be applied.
%
See~\cref{sec:discussion} for features on other platforms.
} that are supported by \codename:


%

% 
\vspace{-0.1cm}
\begin{enumerate}[leftmargin=*,label=\textbullet]
    % \item
    % TrustZone Address Space Controller (TZASC) allows access control over a contiguous memory region (at least 32KB) at the memory bus transaction level by configuring its control registers, which is introduced from TrustZone hardware features~\cite{tzc400}.    
    \item
    Stage-2 Page Table (S2PT), enabled by the virtualization extension, offers a second level of MMU translation which is transparent to the OS.
    %
    It supports page-level memory access control by configuring the corresponding table entry's permission bits~\cite{s2pt}.
    \item \vspace{0.05cm}
    Granule Protection Table (GPT) is an in-memory table structure (like S2PT), from Real Management Extension (RME) of Confidential Computing Architecture (CCA).
    %
    It defines page-level physical memory's accessible CPU states during MMU translation~\cite{rme-extension}.
\end{enumerate}
%

% Depending on the size of the produced logs, switching permissions on larger log buffers (over 4KB) is much more efficient than log copying.
%
We find that switching permissions on log buffers (over 4KB) proves more efficient than log copying.
%
Copying is bound by the size of costly memory-intensive operations that are only efficient for smaller buffers (less than 512B).
% The latter's performance is inherently limited to the size of CPU-intensive copy operations, which only works well on small-size buffers (\eg 256B).
%
Hardware permission switching maintains stable costs by (a) modifying permission control registers or data structures to alter hardware permissions and (b) invalidating stale entries in the translation-lookaside buffer (TLB).
%
This requires significantly less CPU and memory operations.

% Please note that \cref{tab:prot_primitives} only shows the cost of log protection.
% %
% In the real world, this overhead can be amortized (by target system event executions and log generations).


\begin{table}[t]
    \caption{Cost of different memory protection mechanisms.}
    \label{tab:prot_primitives}
    \begin{adjustbox}{width=1\linewidth}
        \setlength{\aboverulesep}{0.0pt}
        \setlength{\belowrulesep}{0.0pt}
        % \setlength{\tabcolsep}{2pt}
        \begin{threeparttable}
        \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Primitive}} & \multicolumn{7}{c}{\textbf{\#CPU cycle\tnote{\textbf{1}}\ cost per log buffer size (less means better)\tnote{3}}}     \\ \cmidrule(lr){2-8}
        & \textbf{64B}  & \textbf{256B} & \textbf{512B} & \textbf{4KB} & \textbf{16KB} & \textbf{32KB} & \textbf{64KB} \\ \midrule
        \textbf{EL3-memcpy} & 1,785 & 2,783 & 4,680 & 24,672 & 98,978 & 198,776 & 400,903 \\
        % \textbf{TZASC}  & {\em 5,352} & {\em 5,352}  & 5,352  & 5,319   & 5,332   & 5,420    \\
        % \rowcolor[gray]{0.85}
        \textbf{S2PT} & {\em 4,482}\tnote{\textbf{2}} & {\em 4,482}\tnote{\textbf{2}} & {\em 4,482}\tnote{\textbf{2}} & 4,482 & 4,496 & 4,516  & 4,636       \\
        % \rowcolor[gray]{0.85}
        \textbf{GPT}  & {\em 4,383}\tnote{\textbf{2}} & {\em 4,383}\tnote{\textbf{2}} & {\em 4,383}\tnote{\textbf{2}} & 4,383 & 4,410 & 4,398  & 4,490       \\ \bottomrule
        \end{tabular}
        \begin{tablenotes}
            % \small
            % \item[\textbf{*}]
            % Detailed system configuration and setup are illustrated in~\cref{sec:impl}.
            \item[\textbf{1}]
            CPU runs at 1.2GHz. Cost of Secure Monitor Call (SMC) context switch round-trip is included.
            %
            Detailed system configuration and setup are illustrated in~\cref{sec:impl}.
            \vspace{0.05cm}
            \item[\textbf{2}]
            S2PT and GPT's protection granularities are at the page level.
            %
            Protecting small-sized buffers will remain at the same cost as protecting a page (4KB).
            \vspace{0.05cm}
            \item[\textbf{3}]
            This only shows {\bf the cost of log protection}.
            %
            In the real world, this overhead can be amortized (by target system event executions and log generations).
        \end{tablenotes}
        \end{threeparttable}
    \end{adjustbox}
    \vspace{-0.4cm}
\end{table}

% \subsubsection{\textbf{Guided TCB and Attack Surface Reduction}}
% \subsubsection{\textbf{\chuqic{High Assurance Secure Log Environment}}}
% \subsection{\textbf{High Assurance Secure Log Environment}}
\subsection{\textbf{High Assurance Log Environment Design}}
\label{subsec:overview_secure_environment}
%
\codename employs a trusted in-memory environment for log protection and management while guaranteeing eventual persistence, but this environment is {\em debloated} by leveraging the three high-assurance strategies.
% 
As~\cref{subfig:overview-hhk} shows, this environment contains a security monitor~({\bf \codename\ Monitor or \sm}) and a protected log daemon~({\bf \codename\ Daemon or \hd}).
% 

The first strategy is to implement the security monitor with only the {\em directly-required} components for log protection.
% 
Specifically, in principle, the monitor only requires control over memory and I/O protection primitives to secure logs~(\cref{subsubsec:security_monitor}).
% 
Other interfaces (e.g., CPU virtualization or code emulation within hypervisors) are not required, thus they are pruned out to avoid vulnerabilities.
%


% \chuqic{As such, the security monitor is desired to be at the management mode (EL3)}
% \chuqic{EL3 here?}

% First, \codename does not rely on large general-purpose components of the virtual machine manager or TrustZone.
% %
% Inspired by security monitor-based approaches~\cite{varun2023omnilog,shepherd2017emlog,dunlap2002revirt}, \codename leverages the privileged system layer.
% %
% However, there is no need to rely on bloated interfaces (of a full-fledged VMM or TrustZone).
% %
% For instance, their interfaces, such as CPU virtualization or code emulation, are not directly required by log protection.
% %
% Thus, \codename only tasks the hardware protection features inside such a layer, to isolate its secure environment from the untrusted OS (\cref{subsubsec:security_monitor}).
% %

The second strategy is to reduce the large software components within the security monitor.
% 
Specifically, a storage device driver is required to persist logs.
%
However, directly porting a commodity driver software into \sm is undesirable---a simple Linux SATA driver has more than 10k lines of code and complex kernel dependencies~\cite{guo2022driverlet}.
%
Thus, \codename employs debloating techniques~\cite{guo2022driverlet,wang2022rttee} to avoid adopting commodity software with large codebases (\cref{subsubsec:debloated_driver}).

% % 
% Note that, in principle, the security monitor can be implemented in any higher privileged layer than the OS, \ie both the hypervisor mode (EL2 in ARM) and system management mode (EL3 in ARM).
% % 
% However, \codename implements the monitor as an EL3 runtime service~\cite{uefi-runtime,atf} for two reasons.
% % 
% First, EL3 has the privilege to control all memory protection primitives (GPT and S2PT).
% % 
% Second, EL3 can be kept small even in enterprise computers that want to run virtual machines, since it would not have to include the hypervisor's TCB. 
% % 
% We discuss virtual machine support in~\autoref{sec:discussion}.
% % 

% Second, only necessarily required software is debloated and ported into the secure environment.
% %
% While the security monitor isolates \codename's environment to keep its integrity, a storage device driver is required for log availability.
% %
% However, directly porting a commodity driver software into \codename increases its complexity.
% %
% For example, a native SATA driver in Linux has more than 10k lines of code, with intrinsic kernel dependencies~\cite{guo2022driverlet}.
% %
% As such, \codename employs debloating techniques~\cite{guo2022driverlet} to avoid adopting commodity software with a large codebase (\cref{subsubsec:debloated_driver}).



% \AD{Don't you also need to save logs using the EL3 (thus, need a device driver)? Be precise.}

% Second, to further keep the secure environment debloated, {\em large buggy codebase of commodity software should not be reused.}

% {\it Third, log management tasks are supported by a protected native daemon on the OS, without using trusted kernels}.\AD{What does this mean?}
The third strategy is to ensure log management through a {\em protected log daemon process} in the untrusted OS.
%
This avoids trusted kernels like Linux and OP-TEE~\cite{optee} used by prior work~\cite{varun2023omnilog,shepherd2017emlog}.
%
% In particular, unlike prior work that manages logs within feature-rich virtual machines, or the TZ secure kernels, \codename directly executes a conventional yet secured log daemon.
% \codename avoids introducing feature-rich VM or trusted kernel management interfaces of prior work~\cite{varun2023omnilog,shepherd2017emlog} into its security monitor.\AD{This seems like it is part of first para.}
%
% A conventional yet secured log daemon is executed.
%
% All required OS services by the log daemon, such as network and scheduling are delegated to the OS~\cite{shinde2017panoply}.
% %
% To achieve secure remote log management, the system administrator establishes a two-way secure authentication channel with the log daemon (\cref{subsec:design_daemon}).
%
While a compromised OS may prevent the scheduling of the log daemon, it is unable to alter the integrity or availability of logs, nor the integrity of log management tasks such as retrieval (\cref{subsubsec:daemon_execution}). 
% A compromised OS can only deny the schedule of the log daemon.
% %
% In other words, it is by no means allowed to tamper with the integrity and availability of protected logs or the integrity of log management tasks like retrieval.
%
% Meanwhile, all tasks should be able to verify that they were completed correctly.


% 
In principle, the monitor can be implemented~(using the first and the second strategy) in any higher privileged layer than the OS, \ie both the hypervisor mode (EL2 in ARM) and system management mode (EL3 in ARM).
% 
However, \codename implements the monitor as an EL3 runtime service~\cite{uefi-runtime,atf} for two reasons.
% 
First, EL3 has the privilege to control all memory protection primitives (including GPT and S2PT) on ARM CPUs, unlike EL2 (only S2PT).
% 
Second, EL3 can be kept small even in enterprise computers that want to run virtual machines, since it would not have to include the hypervisor's TCB. 
% 
We discuss virtual machine support in~\cref{sec:discussion}.
% 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%$
% \subsection{Deployment Model and Assumptions}
\subsection{Deployment Model}
\label{subsec:system_model}

We consider the same enterprise deployment model for \codename as existing research~\cite{varun2023omnilog}.
% 
Specifically, we consider that the enterprise OS vendor (\eg Microsoft, Red Hat Enterprise Linux) will instantiate the monitor (\sm) during system boot~(\cref{subsec:design_security_monitor}).
% 
There is a clear example of this in the past.
% 
In particular, Microsoft Windows 11 instantiates a hypervisor-level monitor during boot-up (for kernel protection), and also enforces firmware-level (UEFI) extensions to support this monitor~\cite{vbs}.
% 
We also consider that the OS vendor will modify the logging facility to invoke \sm for log protection~(\cref{subsec:design_realtime_deadline}) and management.
%
The former exports a protection-aware log function to the administrator, who configures the logs to be collected and protected (\cref{sec:impl}).
% 
The latter include minor changes to retrieve logs remotely using the protected log daemon~(\hd) and locally from audit system tools.
% 
Finally, for remote retrieval~(\cref{subsec:design_daemon}), we assume that the enterprise system administrator will provision cryptographic keys, as is common practice for other IT administration standards like Intel's Active Management Technology~(AMT)~\cite{intel-amt}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Design Challenges}
% \PP{C1: Enforcing protected domains with hardware primitives.}
% %
% The secure environment is kept isolated from the untrusted system.
% %
% Without leveraging general-purpose components like hypervisor or the TrustZone, it is challenging to abstract the domain isolation (memory and device) enforcement from hardware features.

\PP{C1: Reducing software porting and deployment efforts.}
% 
Given strict requirements to ensure high assurance, it is challenging to design an infrastructure where these strategies are satisfied without significant deployment effort (\eg completely rebuilt storage drivers for persistence or natively support the daemon).

% \chuqi{check}

% An observability protection system requires an overhaul of the conventional OS-maintained software infrastructure.
% %
% It is challenging to involve minimal extensions of the conventional software stack and reduce the deployment efforts (\cref{subsec:design_security_monitor}).\adil{your system is making lots of changes to the conventional stack. This will go against you.}
\PP{C2: Enforcing short multi-layer log protection deadlines.}
% 
Unlike prior work that only deals with OS logs, protecting logs from different layers, including applications and network logs, and under the (at least unprivileged) access of an adversary, makes it challenging to enforce uniform and very short deadlines.

\PP{C3: Delegating log management to untrusted OS securely.}
% 
Any task naively delegated to the OS becomes untrustworthy after its compromise. 
% 
Since it is agnostic to administrators when the OS is compromised, the OS can provide completely wrong responses after compromise even without tampering with logs.

==> tex/overview-old.tex <==
\section{\codename Overview}
\label{sec:design_overview}

% Inspired by the limitations of existing solutions, \cref{subfig:overview-hhk} presents the \codename's guide to the fast, secure, and high-assurance observability protection infrastructure.

Considering the limitations of the above existing work (\cref{subsec:limitations_of_existing_protection_solutions}), \codename proposes two key design principles.
% 
First, to achieve high performance and prevent log tampering by strong attackers (overcoming {\bf L1} and {\bf L2}), \codename leverages a memory permission switch mechanism that enables administrators to efficiently protect logs asynchronously within very short, configurable windows~(\cref{subsec:overview_inmemory_observability_protection}).
% 
Second, to ensure logs remain protected in the secure environment with high-assurance (overcoming {\bf L3}), \codename leverages principled strategies to reduce its attack surface and TCB for dedicated secure environments~(\cref{subsec:overview_secure_environment}).
% 

% First, \codename aims to achieve both efficiency and security in log protection, keeping high runtime performance while maintaining a controllable tiny real-time protection window.
%
% First, instead of {\em transmitting} logs to either a privileged memory or a tamper-proof device, \codename employs the memory permission switch for log protection.
% %
% This offers an avenue to rapidly protect a batch of logs in an extremely short time span, enabling the enforcement of a tiny real-time protection window for logs.
% %
% Therefore, \codename\ {\em maintains runtime efficiency with a configurable real-time tiny log protection window, enhancing security.} (\cref{subsec:overview_inmemory_observability_protection}).

% Second, \codename departs from relying on general-purpose layers to hold a secure log environment, instead opting for a dedicated environment built upon the thin system management mode (SMM) layer.
% %
% This excludes all commodity components, delegating non-critical log management tasks to the native OS, under the secure interposition of SMM.
% %
% By doing so, \codename then {\em achieves its principled high assurance secure environment design} (\cref{subsec:overview_secure_environment}).

% 
Given the rising use of ARM in enterprises and cloud computing~\cite{hof2022blackbox}, we use ARM as the reference architecture of the host machine in this paper.
%
We discuss \codename portability to other architectures in~\cref{sec:discussion}.

\subsection{Threat Model and Assumptions}
\label{subsec:threat_model}

Like recent work in log protection~\cite{varun2023omnilog,ahmad2022hardlog,riccardo2020kennylogging,paccagnella2020custos}, we assume the host system is initially benign, but a \textit{non-privileged remote adversary} starts to attack it at time $t_s$.
%
The adversary then exploits software and kernel vulnerabilities in the host system to
(a) circumvent the common defenses~(e.g., ASLR, DEP, and stack canaries) and 
(b) escalate the privilege to the root at time $t_c$. 
%
Being aware of mechanisms of system observability collection, to hide their footprints, the adversary attempts to tamper with the logs in kernel memory or on storage, striving to hide the attack footprints (\ie logs between $t_s$ and $t_c$)~\cite{mitrelinuxlogs,mitrewindowslogs}.
%
Before $t_c$, the observability capturer is honestly deployed inside the OS.
Post-compromise (after $t_c$), an adversary gains full system control and corrupts the observability capture (\eg they can simply stop the in-kernel capturer).
% 
Hence, logs after $t_c$ cannot be trusted and are assumed to be {\em worthless} for forensic analysis~\cite{ahmad2022hardlog}.
%

%
\PP{Assumptions.}
%
We assume IT administrators and vendor-supplied hardware and firmware (BIOS) are trustworthy.
%
In addition, cryptographic protocols and key management work as expected. 
%
Moreover, we assume a secure boot authenticates system configurations and key provisions, ensuring the system's initial state is always benign.
% %
% Specifically, a pair of keys is provisioned by the administrator to set up the secure channel~\cite{ahmad2022hardlog,varun2023omnilog} for remote log management.
% %
% The public key is always securely kept inside the host (\cref{subsec:design_security_monitor}), while the administrator keeps the private key.
% %
% Apart from normal system devices (\eg filesystem and storage), a {\em secondary log storage device} is connected to the host dedicated to log persistence.
%
% Lastly, side-channel attacks are out of the scope of this work.\adil{Is that all that is out-of-scope? Check HardLog/OmniLog.}\chuqi{to be fixed}


\subsection{Background on ARM CPU Features}
\label{sec:arm_background}

\PP{Exception levels (ELs).}
%
Modern ARM CPUs have four exception levels: applications (EL0), the OS (EL1), the hypervisor (EL2), and system management mode (SMM, EL3).
%
Higher ELs are capable of interposing lower ELs (\eg access their memory and system registers).
%
SMM also referred to as the ``secure monitor'', controls essential system resources (\eg interrupt and power management) and provides secure software for the system~\cite{atf} (\eg trusted boot primitives~\cite{cerdeira2020tzsok}).
%
SMM is designed to be small, trustworthy, and verifiable, given its privileged security roles in the system.
% (in fact, only two bugs in SMM have been revealed in recent years~\cite{cerdeira2020tzsok}).
%
The OS can issue a Secure Monitor Call (\textcode{SMC}) to trap into and synchronize SMM for requested services.

\PP{Granule protection table (GPT).}
%
GPT is an in-memory (page-table-like) infrastructure introduced by Realm Management Extension (RME)~\cite{rme-extension} of Confidential Computing Architecture (CCA).
%
CCA introduces four CPU {\em security states}: normal, secure (for TZ secure world), realm (for CCA's confidential VMs~\cite{cca}), and root (exclusively for EL3).
%
It allows dynamically configuring a physical memory granule's (page-level) accessible states ({\em \eg normal, secure, realm, root, all, or none}).
%
Each last-level GPT entry controls up to sixteen physical pages' accessible CPU states~\cite{rme-extension-website}.
%
During the page table walk, RME hardware enforces MMU to perform a granule protection check (GPC) and check the target page's access permission.
%
The GPT's program interface (\ie control register and table edit) is exclusive to SMM.
%
% \chuqi{do we need to introduce CPU's security state (normal, secure, realm, root)? I guess not.}

\subsection{Configurable Real-Time Log Permission Switch}
% 
\label{subsec:overview_inmemory_observability_protection}

\codename leverages {\em permission-switch-based in-memory log protection} using a precise, controlled hardware timer to achieve short real-time deadlines.
% \adil{fix sentence and add memory permission switching idea.}
% 
This approach can inherently provide tighter configurable deadlines than I/O-based protection~\cite{ahmad2022hardlog}, which suffers from large device I/O latencies~(\cref{subsec:limitations_of_existing_protection_solutions}) and are prone to interference from other devices.
% 
The paragraphs below rationalize our approach.
% 


A reliable, periodic hardware timer for log protection allows an administrator to configure a real-time protection delay of $T_p + \epsilon$, where $T_p$ is the timer interrupt frequency and $\epsilon$ is the latency incurred while protecting logs in memory.
% 
Hardware timers today have a high resolution; hence, $T_p$ can be tiny (\eg \textus{100}--\textms{1}).
% 
The value of $\epsilon$ depends (mostly) on the protection mechanism used (discussed below).
% 

% (e.g., copying logs from OS memory to protected regions).
% 
% real-time deadline of $T_p$, each log should be protected in a window of $T_p + \epsilon$, where $\epsilon$ is a negligible, regulated system-induced delay.
% 
% This introduces an unrealistically challenging window for adversaries to perform log tampering attacks.
%
% Such a concept aligns with proposed practices in system hardening solutions, such as continuous code re-randomization~\cite{king2016shuffler}.


%
% I/O-based asynchronous protections like~\cite{ahmad2022hardlog} incur large time windows~(\cref{subsec:limitations_of_existing_protection_solutions}).
% due to the unpredictable I/O latencies.\adil{not really unpredictable. You can predict them as HardLog did.}

% \adil{change}
% %
% Hence, in-memory protection is required to isolate logs fastly.
% %

% Obviously, logs can be batched and transmitted to an in-memory secure environment via memory copy~\cite{varun2023omnilog}.


\codename keeps the value of $\epsilon$ low by leveraging {\em hardware memory permission switch}, instead of the memory copy used by prior work~\cite{varun2023omnilog}.
% 
In particular, the CPU-intensive nature of memory copy makes it very costly when batching logs for real-time protection.
%
To properly illustrate this cost, we compare copying log buffers to EL3 (ARM's most privileged execution level), as used in~\cite{varun2023omnilog}, against protecting them by the following access permission-based techniques:

% , it falls short of a configurable and short real-time deadline (detailed in the following paragraphs).
% %
% Instead, we propose to use permission control by using hardware primitives to restrict the OS' access permission views over log buffers.
% %

% \adil{some minor changes below required. first talk about how the timer allows real-time in this paragraph.}
%
% Essentially, given a real-time deadline of $T_p$, each log should be protected in a window of $T_p + \epsilon$, where $\epsilon$ is a negligible, regulated system-induced delay.
% %
% This introduces an unrealistically challenging window for adversaries to perform log tampering attacks.
% %
% Such a concept aligns with proposed practices in system hardening solutions, such as continuous code re-randomization~\cite{king2016shuffler}.
%
% \adil{Nit: it's not really established until its used in the real-world, continuous code randomization is "proposed".} \chuqi{fixed.}
% 
% To this end, we propose employing in-memory log protection, obviating the inherent latency associated with local or network I/O transmissions.


% 
\begin{enumerate}[leftmargin=*,label=\textbullet]
    \item
    {\em TrustZone Address Space Controller (TZASC)}~\cite{tzc400} allows bus transaction-level access control over a contiguous memory region by configuring its control registers, which is introduced from TrustZone hardware features.
    
    \item \vspace{0.05cm}
    {\em Stage-2 Page Table (S2PT)}~\cite{s2pt}, enabled by virtualization extension, offers a second level of MMU translation which is transparent to the OS.
    %
    It supports page-level memory access control by configuring the corresponding table entry.
    
    \item \vspace{0.05cm}
    {\em Granule Protection Table (GPT)}~\cite{rme-extension}, introduced by RME, which enforces GPC check during MMU translation (\cref{sec:arm_background}).
\end{enumerate}
%

%
\cref{tab:prot_primitives} shows latency results of protecting buffers of different sizes with the aforementioned techniques.
% 
Memory copy consumes significantly more cycles than permission-based primitives, which only require changing permissions in their respective data structures and invalidating stale entries in the translation-lookaside buffer (TLB).
%
In terms of permission-based protection, TZASC lacks the granularity needed for dynamic protection due to its static setup and limited region count~\cite{li2021twinvisor}.
% 
While both S2PT and GPT are ``MMU-table-walk-based'' approaches, GPT is slightly more efficient.
% 
GPT permits one last-level entry to set permissions for 16 pages at once~\cite{rme-extension-website}, whereas S2PT requires a per-page permission setting.
% 
Therefore, GPT needs fewer table walks and invalidations for table entries, particularly when modifying permissions for large memory sizes~(\eg 1 MB).
%
Moreover, S2PT is typically adopted in virtualization-enabled systems, which causes extra performance tax~\cite{zhou2023coreslicing}.
%
% The quick switchability of memory permissions allows us to employ a hardware timer: by switching the log buffer's permission at a frequency $T_p$, each log can be protected within a configurable window of $T_p$, plus a negligible delay $\epsilon$ caused by the small overhead of permission change.

\begin{table}[t]
    \caption{CPU cycle cost for different memory protections.}
    \label{tab:prot_primitives}
    \begin{adjustbox}{width=1\linewidth}
        \setlength{\aboverulesep}{0.0pt}
        \setlength{\belowrulesep}{0.0pt}
        % \setlength{\tabcolsep}{2pt}
        \begin{threeparttable}
        \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Primitive}\tnote{\textbf{*}}} & \multicolumn{5}{c}{\textbf{\#CPU cycle\tnote{\textbf{1}} cost per log buffer size (less means better)}}     \\ \cmidrule(lr){2-6}
        & \textbf{4KB} & \textbf{64KB} & \textbf{256KB} & \textbf{512KB} & \textbf{1MB}  \\ \midrule
        \textbf{EL3-memcpy} & 24,672 & 400,903 & 1,583,316 & 3,215,020  & 6,475,735  \\
        \textbf{TZASC}   & N/A   & 5,352  & 5,319   & 5,332   & 5,420    \\
        \textbf{S2PT}   & 4,482  & 4,636  & 4,996   & 5,794   & 7,084    \\
        \rowcolor[gray]{0.85}
        \textbf{GPT} &\textbf{4,383} &\textbf{4,490} &\textbf{4,735}&\textbf{4,814}&\textbf{4,927}\\ \bottomrule
        \end{tabular}
        \begin{tablenotes}
            % \small
            \item[\textbf{*}]
            Detailed system configuration and setup are illustrated in~\cref{sec:impl}.
            \item[\textbf{1}]
            CPU runs at 1.2GHz; The context switch (\textcode{SMC}) cost is included.
        \end{tablenotes}
        \end{threeparttable}
    \end{adjustbox}
\end{table}

% In addition to having the smallest permission change latency ($\epsilon$), GPT offers the following advantages in terms of flexibility and security assurance when compared to other techniques.
% % 
% First, 
% % 
% Second, S2PT is used and can be configured by hypervisors in already virtualized ARM systems for VM isolation, complicating its use without expanding the attack surface (as stated in~\cref{subsec:limitations_of_existing_protection_solutions}).
% % 
% % Third, GPT is intentionally to serve ARM's confidential VM manager for realm world, which is complementary to our adoption without compatibility issues (explained in Sec.X), avoiding shared attack surface with the VMM or other components~\cite{zhang2023shelter,sridhara2023acai}.
% \adil{I would talk about the cost of virtualization itself, instead of this. Don't mix: your next section is about attack surface, not this one.}
% \chuqi{what about a system like BlackBox? use S2PT without virtualization}\adil{Using S2PT means more page table walks (which can slow down computations) even if you don't use VMs. Cite core-slicing.}

In conclusion, \codename uses GPT for efficient and real-time deadline-enforced in-memory log protection.

\subsection{High-Assurance Environment Strategies}
\label{subsec:overview_secure_environment}

% \adil{Not sure about heading yet. Let's keep brainstorming. :) }
% \chuqi{But where should we introduce the "principled" + topdown? this is an overview section.}
% \chuqi{Still failed to write a good overview, sigh. :( }\adil{that's okay.}

% \adil{Focus on three principles here. Keep this short.\\
% 
% {\bf 1st principle:} Avoid sharing software stack with large general-purpose components (e.g., hypervisor/OPTEE), because it increases the attack surface.\\
% %
% {\bf 2nd principle:} Keep the software stack of the log protection environment small and don't reuse any buggy software from existing stacks (e.g., Linux/U-Boot device drivers). This ensures your system has fewer bugs.\\
% % 
% {\bf 3rd principle:} Isolate log {\em management} tasks into an OS-controlled environment, unlike OmniLog that relies on trusted kernels. This ensures your system has fewer bugs due to smaller codebase.\\
% % 
% With the 3rd principle, you can explain the properties that you care about (i.e., remote log retrieval and parsing only when the OS cooperates).
% }
% \adil{protection and management, differentiate these two aspects here.}

% \chuqi{I think the ideas of 2nd and 3rd are like: If some functions should be in TCB, it should be debloated and easy to verify (2nd); If something is unnecessary to be in TCB, they should not be in (3rd).}

% \adil{Top-down again. Start from the principle. Don't make the principle hide in the middle of the para. :)}\chuqi{fixed}

% \adil{I wonder somewhere here whether we should mention our design is inspired by OmniLog, with three key differences/approaches to ensure high-assurance.}

% A secure environment is required to be dedicated to secure log management with a small attack surface (\textbf{G2}) and easy-to-deploy (\textbf{G3}).
%
% To achieve this, there are three key principles, which we discuss in the rest of the section.
% \begin{enumerate}[leftmargin=*]
%     \item [(1)]
%      The log protection mechanisms should not rely on large general-purpose components (\eg hypervisor) to avoid large attack surfaces with other system components.
    
%     \vspace{0.05cm}
%     \item [(2)]
%     The log protection environment software stack should be kept small, avoiding reusing any large buggy software from existing stacks and including them to the TCB.
    
%     \vspace{0.05cm}
%     \item [(3)] 
%     Further extending (2), the log management tasks should be natively supported by but isolated from the OS, instead of using extra runtime (\eg a trusted kernel) in the TCB.
% \end{enumerate}

%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

% \codename constructs its secure environment by (a) only holding and debloating crucial protection mechanisms, including GPT for memory isolation and a protected driver for device isolation, inside a privileged {\em security monitor} (\sm), while (b) delegating the support for a non-crucial log daemon (\hd) to the native OS.

\codename's secure environment design is inspired by {\em privileged-monitor-based} solutions~\cite{varun2023omnilog,shepherd2017emlog}---containing a privileged security monitor ({\bf \codename Monitor, \sm}), a log managing daemon {(\bf \codename Daemon, \hd}), and a {\bf secondary protected log storage device}---but with {\em three key strategies to reduce the environment's attack surface and TCB}.
% 
The rest of this section describes these strategies.
% 

% Instead of relying on common layers and trusted kernels, \codename constructs a secure environment including (a) a {\em privileged security monitor} (\sm) that configures protection mechanisms to maintain the secure environment, (b) a secondary log storage device to persist logs, and (c) a secure log daemon (\hd) which is delegated to be supported by the native OS.
% %
% The following paragraphs illustrate the principles of this approach. 
% %

% {\em First, \codename secure environment does not rely on large general-purpose components (\eg VMM and TZ, along with their respective trusted kernels).}
{\em \uppercase\expandafter{\romannumeral1}. To reduce the attack surface, none of \codename's trusted components are shared with large existing system components (\eg VMM and TZ).}
%
Instead, \codename employs the privileged EL3 (SMM) for \sm alongside a {\em native but secured user-space} daemon for \hd (\cite{varun2023omnilog,shepherd2017emlog} use commodity trusted kernels).
% 
Unlike VMMs and TZ, EL3 is purposefully kept very small (\cref{sec:arm_background}), and provides a narrow interface (through \textcode{SMC}s) to the OS. 
% 
The \hd is designed to only accept remote input through a narrow memory-based communication channel that is secured end-to-end (using cryptographic protocols) with the administrator~(\cref{subsec:design_security_monitor}).
% 
Apart from that, the handling of the user-space daemon is securely delegated to the untrusted OS to keep its codebase small (please refer to the third strategy).
% 

{\em \uppercase\expandafter{\romannumeral2}. To avoid reusing the large buggy codebase of commodity software within its trusted components, \codename leverages debloating.}
%
Besides a trusted kernel, the largest buggy component of an in-memory secure environment is its storage driver.
%
Such a protected driver is required in the privileged \sm, ensuring log persistence.
%
Instead of porting a huge commodity driver into \sm, \sm employs a debloated driver synthesized through {\em driver record-and-replay}~\cite{guo2022driverlet,wang2022rttee}, by automatically recording a driver template through sample I/O tasks and replaying it inside \sm.
%
While there are other choices, like porting and isolating a driver into \sm via memory-safe language, we choose the driver record-and-replay due to (a) easy-of-verification given such a debloated driver, and (b) easy-to-deploy as it can be automatically recorded (explained in \cref{subsec:design_offline}).
%
Nonetheless, the other approaches can be applied as well in the future.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

{\em \uppercase\expandafter{\romannumeral3}. To keep the TCB small with a simple software stack, \codename securely delegates the log daemon's runtime support to the native OS.}
%
The daemon (\hd) must be scheduled and requires networking services to communicate with remote administrators, but it cannot do so itself since it is in userspace.
% 
\codename does not emulate these services within \sm or deploy a trusted kernel~\cite{shepherd2017emlog,varun2023omnilog}, which increases its TCB considerably.
%
Instead, these services are delegated to the OS while interposed by \sm to ensure the integrity of \hd and network communication~(\cref{subsec:design_daemon}).
% 
% The daemon (\hd) process scheduling and system services (\eg network) are transparently supported by the native OS, while \sm 
% protect it from the OS (\ie the untrusted OS is by no means allowed to access the daemon's memory space in any event).
% %
This aligns with the concept of {\em delegate-rather-than-emulate}~\cite{shinde2017panoply,hofmann2013inktag,hof2022blackbox,zhang2023shelter}, preventing expanding the TCB.
%
An organic byproduct of this approach is obviating the resource consumption associated with additional runtimes, such as the performance tax of a VM~\cite{ahmad2022hardlog} or OP-TEE kernel~\cite{optee-overhead}.
%

Although a compromised OS can kill the delegated \hd, deny the network services, pause the timer, or simply halt log capture, it cannot harm the integrity and availability of protected logs.
%
This is because (a) the secure environment and protected logs retain their integrity under the interposition of the \sm; (b) all protected logs will be persisted in secure storage, with their physical availability guaranteed by the \sm protected device driver; and (c) logs created post-OS compromise are deemed worthless~(\cref{subsec:threat_model})~\cite{ahmad2022hardlog,varun2023omnilog}, 
negating the need for service support.\adil{Needs some work.}

\adil{Change overview into principles.}

% \begin{conclusionbox}
% {\bf Takeaway:}
% %
% {\em The secure environment should be kept small and avoid sharing attack surfaces with common components. 
% %
% Critical functions, including memory protection primitives for integrity and a protected storage driver for availability, should be kept debloated inside the environment.
% %
% Non-critical management functions (\ie the log daemon) should be securely delegated to the OS. 
% }
% \end{conclusionbox}
% \chuqi{TODO: use bullet points at the beginning of this section?}
%


==> tex/overview-old1.tex <==
\section{Design Principles}
\label{sec:design_overview}

% Inspired by limitations of the existing work (\cref{subsec:limitations_of_existing_protection_solutions}), this section describes two key design principles of our system, \codename.
% % 
% Given the rising use of ARM-based computers in enterprises and cloud computing, we use ARM as the reference architecture.
% % , where the related features are described in~\cref{sec:arm_background}.
% %
% We discuss \codename's portability to other architectures in~\cref{sec:discussion}.

% Inspired by the limitations of existing work, we propose \codename.
%
In this work, we present \codename, an efficient, secure observability protection system within the high assurance environment.
%
Inspired by the limitations of existing solutions and the privileged security monitor-based protection approaches~\cite{varun2023omnilog,shepherd2017emlog,dunlap2002revirt}, \cref{subfig:overview-hhk} presents the high-level architecture of \codename.
%

%
Two key design principles are applied for efficient and secure log protection and management.
%
First, each log, after generation, {\em is protected in memory in an enforced short real-time deadline by swift memory permission switches}~(\cref{subsec:overview_inmemory_observability_protection}), before finally being persisted.
%
Second, a dedicated secured environment manages logs at runtime.
%
{\em It does not rely on bloated general-purpose components, and log management tasks are natively delegated to the OS}~(\cref{subsec:overview_secure_environment}).

% In this section, we illustrate the aforementioned design principles~(\cref{subsec:design_principles}) and \codename's deployment system model (\cref{subsec:system_model}).
%
Given the rising use of ARM-based computers in enterprises and cloud computing, we use ARM as the reference architecture.
% , where the related features are described in~\cref{sec:arm_background}.
%
We discuss \codename's portability to other architectures in~\cref{sec:discussion}.

% \subsection{Preliminaries of ARM CPU Features}
% \subsection{Design Principles}
% \label{subsec:design_principles}


% \subsubsection{Configurable Deadline-Enforced In-Memory Log Permission Switch}
% \subsubsection{\textbf{Configurable Deadline-Enforced In-Memory Log Permission Switch}}
\subsection{\textbf{Configurable Deadline-Enforced In-Memory Log Permission Switch}}
% 
\label{subsec:overview_inmemory_observability_protection}
% \AD{The heading style looks ugly tbh.}

To achieve high performance while preventing strong attackers from tampering with logs (overcoming {\bf L1} and {\bf L2}),
% 
logs should be protected in memory by swift permission switches, within short real-time deadlines set by administrators.
% 

% {
% in memory inhertly tight deadlines but performance
% -> intuitively 
% + permission switch
% 
% }

In-memory protection can inherently provide tighter deadlines than I/O-based protection~\cite{ahmad2022hardlog}, which suffers from large device latencies~(\cref{subsec:limitations_of_existing_protection_solutions}) and interference from other devices.
% 
% \AD{Not a good word, rephrase}
% Straightforwardly, logs are copied from the OS to the protected memory~\cite{varun2023omnilog}.\AD{This entire sentence seems to say the same thing as the first one in the para.}
In such protection settings, logs are copied from the OS to the protected memory~\cite{varun2023omnilog}.
%
However, short protection deadlines result in highly frequent log protections with slow memory copy, which is time-consuming.


% Given the log throughput (\cref{tab:obs_throughput}), frequently copying logs between domains may introduce non-negligible overheads~\cite{}.
% \adil{Not clear what you want to say in that second sentence.}\chuqi{to hint the overhead?}

%
%
To efficiently protect logs, switching their access permissions by hardware permission primitives can mitigate the large memory-copy overhead.
%
% Intuitively, using memory permission switches to protect logs avoids the time-consuming large amount of data copy, which can improve efficiency.
% ~\cite{du2019xpc, elphinstone2013l3tol4}\AD{These cites look like the idea is already used for logs.}.  
%
% This intuition is derived by adopting zero-copy temporary permission mapping for message passing optimization~\cite{du2019xpc, elphinstone2013l3tol4}.
%
To understand this, \cref{tab:prot_primitives} compared copying log buffers to the privileged system layer (EL3), against protecting them using hardware memory permission primitives ({\bf \hpp}\footnote{
TrustZone Address Space Controller (TZASC~\cite{tzc400}) is an alternative memory permission primitive controlled by EL3.
%
Its static setup and limited region count~\cite{li2021twinvisor} lacks flexibility.
%
Thus, we discuss, design, and implement \codename via S2PT and GPT. 
%
See discussion in~\cref{sec:discussion} to understand their implications and features on other platforms.
}):


%

% 
\begin{enumerate}[leftmargin=*,label=\textbullet]
    % \item
    % TrustZone Address Space Controller (TZASC) allows access control over a contiguous memory region (at least 32KB) at the memory bus transaction level by configuring its control registers, which is introduced from TrustZone hardware features~\cite{tzc400}.
    
    \item \vspace{0.05cm}
    Stage-2 Page Table (S2PT), enabled by the virtualization extension, offers a second level of MMU translation which is transparent to the OS.
    %
    It supports page-level memory access control by configuring the corresponding table entry's permission bits~\cite{s2pt}.
    
    \item \vspace{0.05cm}
    Granule Protection Table (GPT) is an in-memory table structure (like S2PT), from Real Management Extension (RME) of Confidential Computing Architecture (CCA).
    %
    It defines page-level physical memory's accessible CPU states for MMU translation~\cite{rme-extension}.
\end{enumerate}
%

% Depending on the size of the produced logs, switching permissions on larger log buffers (over 4KB) is much more efficient than log copying.
%
We find that switching permissions on log buffers (over 4KB) proves significantly more efficient than log copying.
%
Copying is bound by the size of costly memory-intensive operations that are only efficient for smaller buffers (\eg 256B).
% The latter's performance is inherently limited to the size of CPU-intensive copy operations, which only works well on small-size buffers (\eg 256B).
%
Permission switches maintain stable overheads by (a) modifying interfaces and data structures to alter hardware permissions (at the page level) and (b) invalidating stale entries in the translation-lookaside buffer (TLB).

%
% Note that the runtime (future) impact of TLB flushing on computations is not insignificant, but our runtime evaluation (\cref{subsec:performance_evaluation}) still illustrates significant benefits of permission switch over memory copy.
% Generally, permission switches maintain a stable overhead by (a) modifying their interfaces and data structures to change hardware permissions and (b) invalidating stale entries in the translation-lookaside buffer (TLB).
%

% \AD{Can we just remove this permission switch feature from here? You may add your footnote-1 here saying that TZASC does not support flexible permission changes.}\chuqi{check}

% \AD{Still not clear. Can you plainly say something like "memcpy as a means of protection used by prior work is too slow, and this is our proof."?}\chuqi{check}

% \AD{Not a good start because readers will not be thinking about permission switch. You can say something like "One way to avoid XYZ is using memory permission switch .."} \chuqi{check}

% \AD{Simplify a bit and be more precise as to why memcpy is faster in <4KB.}\chuqi{check}

% \adil{I feel like you want to say something about what techniques your system can use (i.e., S2PT and GPT) and what makes these better than memcpy/TZASC.}\chuqi{Mentioned in Sec. 5.1.}

% given the amount of data, due to the time-consuming data-copy nature.

% only require changing permissions in their respective data structures and invalidating stale entries in the translation-lookaside buffer (TLB)

% Memory copy consumes significantly more cycles than permission-based primitives, which only require changing permissions in their respective data structures and invalidating stale entries in the translation-lookaside buffer (TLB).
% % 
% Specifically, even for smaller buffer sizes like 4KB, memory copy is $\sim6\times$ slower.
% % 
% As expected, it gets progressively worse with larger buffer sizes.
% % 
% Note that the runtime (future) impact of TLB flushing on computations is not insignificant, but our runtime evaluation~(\cref{sec:performance_evaluation}) still illustrates significant benefits of permission switch over memory copy.



% In terms of permission-based protection, TZASC lacks the granularity needed for dynamic protection due to its static setup and limited region count~\cite{li2021twinvisor}.
% % 
% While both S2PT and GPT are ``MMU-table-walk-based'' approaches, GPT is slightly more efficient.
% % 
% GPT permits one last-level entry to set permissions for 16 pages at once~\cite{rme-extension-website}, whereas S2PT requires a per-page permission setting.
% % 
% Therefore, GPT needs fewer table walks and invalidations for table entries, particularly when modifying permissions for large memory sizes~(\eg 1 MB).
% %
% Moreover, S2PT is typically adopted in virtualization-enabled systems, which causes extra performance tax~\cite{zhou2023coreslicing}.
%
% The quick switchability of memory permissions allows us to employ a hardware timer: by switching the log buffer's permission at a frequency $T_p$, each log can be protected within a configurable window of $T_p$, plus a negligible delay $\epsilon$ caused by the small overhead of permission change.


\begin{table}[t]
    \caption{Cost of different memory protection mechanisms.}
    \label{tab:prot_primitives}
    \begin{adjustbox}{width=1\linewidth}
        \setlength{\aboverulesep}{0.0pt}
        \setlength{\belowrulesep}{0.0pt}
        % \setlength{\tabcolsep}{2pt}
        \begin{threeparttable}
        \begin{tabular}{lccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Primitive}\tnote{\textbf{*}}} & \multicolumn{6}{c}{\textbf{\#CPU cycle\tnote{\textbf{1}}\ cost per log buffer size (less means better)}}     \\ \cmidrule(lr){2-7}
        & \textbf{256B} 
        & \textbf{4KB} & \textbf{32KB} & \textbf{64KB} & \textbf{128KB} & \textbf{256KB}  \\ \midrule
        \textbf{EL3-memcpy} & 2,783 & 24,672 & 198,776 & 400,903 & 811,658  & 1,583,316  \\
        % \textbf{TZASC}  & {\em 5,352} & {\em 5,352}  & 5,352  & 5,319   & 5,332   & 5,420    \\
        % \rowcolor[gray]{0.85}
        \textbf{S2PT}   & {\em 4,482}\tnote{\textbf{2}} & 4,482  & 4,516  & 4,636   & 4,712   & 4,996    \\
        % \rowcolor[gray]{0.85}
        \textbf{GPT}    & {\em 4,383}\tnote{\textbf{2}} & 4,383  & 4,398  & 4,490   & 4,514   & 4,735    \\ \bottomrule
        \end{tabular}
        \begin{tablenotes}
            % \small
            \item[\textbf{*}]
            Detailed system configuration and setup are illustrated in~\cref{sec:impl}.
            \item[\textbf{1}]
            CPU runs at 1.2GHz; cost of the context switch (SMC) round-trip is included.
            \item[\textbf{2}]
            S2PT and GPT's protection granularities are at the page level.
            %
            Protecting a single log entry (256B) will remain the same cost as protecting a page (4KB).
            % \AD{You need to explain why 256B and 4KB times remain the same for TZASC, etc.}
        \end{tablenotes}
        \end{threeparttable}
    \end{adjustbox}
\end{table}
% \begin{table}[t]
%     \caption{Cost of different memory protection mechanisms.}
%     \label{tab:prot_primitives}
%     \begin{adjustbox}{width=1\linewidth}
%         \setlength{\aboverulesep}{0.0pt}
%         \setlength{\belowrulesep}{0.0pt}
%         % \setlength{\tabcolsep}{2pt}
%         \begin{threeparttable}
%         \begin{tabular}{lccccccc}
%         \toprule
%         \multirow{2}{*}{\textbf{Primitive}\tnote{\textbf{*}}} & \multicolumn{6}{c}{\textbf{\#CPU cycle\tnote{\textbf{1}}\ cost per log buffer size (less means better)}}     \\ \cmidrule(lr){2-7}
%         & \textbf{256B} 
%         & \textbf{4KB} & \textbf{64KB} & \textbf{256KB} & \textbf{512KB} & \textbf{1MB}  \\ \midrule
%         \textbf{EL3-memcpy} & 2,783 & 24,672 & 400,903 & 1,583,316 & 3,215,020  & 6,475,735  \\
%         % \textbf{TZASC}  & {\em 5,352} & {\em 5,352}  & 5,352  & 5,319   & 5,332   & 5,420    \\
%         % \rowcolor[gray]{0.85}
%         \textbf{S2PT}   & {\em 4,482}\tnote{\textbf{2}} & 4,482  & 4,636  & 4,996   & 5,794   & 7,084    \\
%         % \rowcolor[gray]{0.85}
%         \textbf{GPT}    & {\em 4,383}\tnote{\textbf{2}} & 4,383  & 4,490  & 4,735   & 4,814   & 4,927    \\ \bottomrule
%         \end{tabular}
%         \begin{tablenotes}
%             % \small
%             \item[\textbf{*}]
%             Detailed system configuration and setup are illustrated in~\cref{sec:impl}.
%             \item[\textbf{1}]
%             CPU runs at 1.2GHz; cost of the context switch (SMC) round-trip is included.
%             \item[\textbf{2}]
%             S2PT and GPT's protection granularities are at the page level.
%             %
%             Protecting smaller buffers (256B) will remain the same cost as protecting a page (4KB).
%             % \AD{You need to explain why 256B and 4KB times remain the same for TZASC, etc.}
%         \end{tablenotes}
%         \end{threeparttable}
%     \end{adjustbox}
% \end{table}


% \subsubsection{\textbf{Guided TCB and Attack Surface Reduction}}
% \subsubsection{\textbf{\chuqic{High Assurance Secure Log Environment}}}
\subsection{\textbf{\chuqic{High Assurance Secure Log Environment}}}
\label{subsec:overview_secure_environment}
% %

To realize in-memory protection~(\cref{subsec:overview_inmemory_observability_protection}), \codename must also leverage an in-memory secure environment.
% 
However, this environment is designed with the following strategies to systematically reduce bloated interfaces and attack surface (overcoming {\bf L3}).
% 

% \codename is inspired by privileged security-monitor-based protections~\cite{shepherd2017emlog,varun2023omnilog,ahmad2024veil}.
% %
% To avoid sharing general-purpose components' bloated interfaces and attack surfaces (overcoming {\bf L3}), logs should be managed within a dedicated secure environment with high assurance.
% %
% We explain the required strategies in the following.
% %

% \AD{Not a great heading.}
% \AD{Better to introduce the security monitor later (e.g., 4.1.2)}
% \chuqi{Can you help a bit with the heading?}

{\em Any components within the secure environment should not be shared with large general-purpose system components.}
%
Specifically, a privileged security monitor is required to task only with maintaining system domain isolation (\ie memory and device), which keeps the high assurance secure log environment.
% \AD{This is not the correct use of ", which". ", which" is used to explain the property of something.}
%
Preferably, it is to be deployed at the management mode (EL3 privilege level), as a runtime service within the secure firmware~\cite{atf}.
%
This benefits from the EL3's privilege to control fundamental system resources (we further discuss alternative security monitor design choices in \cref{sec:discussion}).
%


\AD{Don't you also need to save logs using the EL3 (thus, need a device driver)? Be precise.}

% Second, to further keep the secure environment debloated, {\em large buggy codebase of commodity software should not be reused.}

Second, {\em log management tasks should be securely delegated to the OS without using trusted kernels}.
%
This avoids introducing feature-rich VM or trusted kernel management functionality of prior work into the security monitor.
% This further circumvents heavy interfaces associated with feature-rich VMs or the TZ kernels.\AD{Not the precise sentence. You can say something like "This avoids introducing complex virtual machine or trusted kernel management functionality of prior work into the security monitor."}
%
Ideally, a conventional yet secured log daemon should be tasked to manage logs.
%
All required OS services by the log daemon, such as network, execution runtime, and scheduling should be securely delegated to the OS~\cite{shinde2017panoply}.
%
While a compromised OS may prevent the scheduling of the log daemon, it must not alter the integrity or availability of the logs, nor the integrity of log management tasks such as retrieval. 
% A compromised OS can only deny the schedule of the log daemon.
% %
% In other words, it is by no means allowed to tamper with the integrity and availability of protected logs or the integrity of log management tasks like retrieval.
%
Meanwhile, all tasks should be able to verify that they were completed correctly.



% Like recent work~\cite{varun2023omnilog,ahmad2022hardlog}, \codename considers the deployment under an enterprise model, including (a) the enterprise system software vendor, (b) the IT administrator, and (c) the host machine.


% \PP{System software vendors}
% %
% They extend the system software (\eg OS and privileged firmware)\AD{I see you misuse the \eg and \ie very often. Please check the correct usage of these terms.} to support the components required by \codename.
% %
% This practice is similar to commercial enterprise OS projects.
% %
% For instance, Red Hat Enterprise Linux~\cite{redhat} extends the OS to support flexible subsystems (\eg Auditd~\cite{auditd} for audit logs),
% %
% % pKVM~\cite{} extends the hypervisor enforcement of access-control restrictions on host;\AD{Why is this relevant here? You're not asking for hypervisor changes.} 
% and firmware projects like CLIENTPC~\cite{clientpc} develop OS-compliant UEFI (\eg supports different major client OSs in ARM).
% \AD{You need to be precise as to what components are needed, etc. It might be better to explain after design.}

% \AD{It may be better to write this section like: "We need XYZ at YYZ and this is how it will work". That is more simpler and less threatening.}

% %
% \PP{IT administrators} They provision the enterprise machine before being deployed and actively manage the machine during runtime.
% %
% During machine provisioning, they install \codename system software components into the machine.
% %
% They either use \codename's provided log daemon or the OS-native daemon\AD{Can HHK support the native daemon?} but install required attestation keys (\cref{subsubsec:daemon_execution}).
% %
% Required certificates and cryptographic keys are provisioned to the machine (\ie Intel AMT~\cite{intel-amt} practices), to support runtime secure communication channels (\cref{subsec:design_daemon}).

==> tex/overview-sp.tex <==
% \section{Design Principles}
\section{\codename Overview}
\label{sec:design_overview}

Inspired by limitations of the existing work (\cref{subsec:limitations_of_existing_protection_solutions}), this section describes two key design principles of our system, \codename.
% 
Given the rising use of ARM-based computers in enterprises and cloud computing, we use ARM as the reference architecture.
% , where the related features are described in~\cref{sec:arm_background}.
%
We discuss \codename's portability to other architectures in~\cref{sec:discussion}.



% \subsection{Preliminaries of ARM CPU Features}


\subsection{Configurable {\em In-Memory} Deadline-Enforced Log Protection}
% 
\label{subsec:overview_inmemory_observability_protection}

To achieve high performance while preventing strong attackers from tampering with logs (overcoming {\bf L1} and {\bf L2}),
% 
we propose that {\em logs should be fastly protected in memory within tight deadlines set by system administrators}.
% 

% {
% in memory inhertly tight deadlines but performance
% -> intuitively 
% + permission switch
% 
% }

In-memory protection can inherently provide tighter deadlines than I/O-based protection~\cite{ahmad2022hardlog}, which suffers from large device latencies~(\cref{subsec:limitations_of_existing_protection_solutions}) and interference from other devices.
% 
% In addition, hardware permission switch mechanisms---which simply change permissions on memory using their control interfaces---can also significantly shorten protection deadlines and improve overall system performance, compared to simply copying logs to a secure environment.
%
\chuqic{
Despite their promise, tight protection deadlines result in highly frequent log protections (\ie passing logs between untrusted and trusted domains).
%
Given the log throughput (\cref{tab:obs_throughput}), frequently copying logs between domains may introduce non-negligible overheads~\cite{}.
}\adil{Not clear what you want to say in that second sentence.}

\chuqic{
%
Intuitively, using temporary permission switches to protect logs avoids the time-consuming large amount of data copy, which can improve efficiency~\cite{du2019xpc, elphinstone2013l3tol4}.  
%
% This intuition is derived by adopting zero-copy temporary permission mapping for message passing optimization~\cite{du2019xpc, elphinstone2013l3tol4}.
%
To understand this, \cref{tab:prot_primitives} compared copying log buffers to the privileged system layer (EL3), against protecting them using hardware permission primitives (\hpp):
}


%

% 
\begin{enumerate}[leftmargin=*,label=\textbullet]
    \item
    {\em TrustZone Address Space Controller (TZASC)} allows access control over a contiguous memory region (at least 32KB) at the memory bus transaction level by configuring its control registers, which is introduced from TrustZone hardware features~\cite{tzc400}.
    
    \item \vspace{0.05cm}
    {\em Stage-2 Page Table (S2PT)}, enabled by virtualization extension, offers a second level of MMU translation which is transparent to the OS.
    %
    It supports page-level memory access control by configuring the corresponding table entry's permission bits~\cite{s2pt}.
    
    \item \vspace{0.05cm}
    {\em Granule Protection Table (GPT)} is a page-table-like in-memory structure (similar to S2PT)\adil{this may be confusing. It's not really like page tables. Rephrase.}, from Real Management Extension (RME) of Confidential Computing Architecture (CCA).
    %
    It defines page-level physical memory granules’ accessible CPU states~\cite{rme-extension}.
\end{enumerate}
%

Depending on the size of the produced logs, switching permissions on larger log buffers (over 4KB) is much more efficient than log copying.
%
Generally, permission switches maintain a stable overhead by programming the control interfaces to (a) modify their respective data structures to change hardware permissions and (b) invalidate stale entries in the translation-lookaside buffer (TLB).
%
Conversely, memory copy is preferable for small logs (less than 1KB) as its overhead linearly increases with the volume of logs, due to the inherent time demands for copying.

\adil{I feel like you want to say something about what techniques your system can use (i.e., S2PT and GPT) and what makes these better than memcpy/TZASC.}

% given the amount of data, due to the time-consuming data-copy nature.

% only require changing permissions in their respective data structures and invalidating stale entries in the translation-lookaside buffer (TLB)

% Memory copy consumes significantly more cycles than permission-based primitives, which only require changing permissions in their respective data structures and invalidating stale entries in the translation-lookaside buffer (TLB).
% % 
% Specifically, even for smaller buffer sizes like 4KB, memory copy is $\sim6\times$ slower.
% % 
% As expected, it gets progressively worse with larger buffer sizes.
% % 
% Note that the runtime (future) impact of TLB flushing on computations is not insignificant, but our runtime evaluation~(\cref{sec:performance_evaluation}) still illustrates significant benefits of permission switch over memory copy.



% In terms of permission-based protection, TZASC lacks the granularity needed for dynamic protection due to its static setup and limited region count~\cite{li2021twinvisor}.
% % 
% While both S2PT and GPT are ``MMU-table-walk-based'' approaches, GPT is slightly more efficient.
% % 
% GPT permits one last-level entry to set permissions for 16 pages at once~\cite{rme-extension-website}, whereas S2PT requires a per-page permission setting.
% % 
% Therefore, GPT needs fewer table walks and invalidations for table entries, particularly when modifying permissions for large memory sizes~(\eg 1 MB).
% %
% Moreover, S2PT is typically adopted in virtualization-enabled systems, which causes extra performance tax~\cite{zhou2023coreslicing}.
%
% The quick switchability of memory permissions allows us to employ a hardware timer: by switching the log buffer's permission at a frequency $T_p$, each log can be protected within a configurable window of $T_p$, plus a negligible delay $\epsilon$ caused by the small overhead of permission change.

\begin{table}[t]
    \caption{Cost of different memory protection mechanisms.}
    \label{tab:prot_primitives}
    \begin{adjustbox}{width=1\linewidth}
        \setlength{\aboverulesep}{0.0pt}
        \setlength{\belowrulesep}{0.0pt}
        % \setlength{\tabcolsep}{2pt}
        \begin{threeparttable}
        \begin{tabular}{lccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Primitive}\tnote{\textbf{*}}} & \multicolumn{6}{c}{\textbf{\#CPU cycle\tnote{\textbf{1}} cost per log buffer size (less means better)}}     \\ \cmidrule(lr){2-7}
        & \textbf{\chuqic{256B}} 
        & \textbf{4KB} & \textbf{64KB} & \textbf{256KB} & \textbf{512KB} & \textbf{1MB}  \\ \midrule
        \rowcolor[gray]{0.85}
        \textbf{EL3-memcpy} & \chuqic{2,783} & 24,672 & 400,903 & 1,583,316 & 3,215,020  & 6,475,735  \\
        \textbf{TZASC}  & {\em 5,352} & {\em 5,352}  & 5,352  & 5,319   & 5,332   & 5,420    \\
        \textbf{S2PT}   & {\em 4,482} & 4,482  & 4,636  & 4,996   & 5,794   & 7,084    \\
        \textbf{GPT}    & {\em 4,383} & 4,383  & 4,490  & 4,735   & 4,814   & 4,927    \\ \bottomrule
        \end{tabular}
        \begin{tablenotes}
            % \small
            \item[\textbf{*}]
            Detailed system configuration and setup are illustrated in~\cref{sec:impl}.
            \item[\textbf{1}]
            CPU runs at 1.2GHz; the context switch (SMC) round-trip cost is included.
        \end{tablenotes}
        \end{threeparttable}
    \end{adjustbox}
\end{table}


\subsection{Guided TCB and Attack Surface Reduction}
\label{subsec:overview_secure_environment}

To ensure logs are protected with high assurance (overcoming {\bf L3}),
% 
we propose the following strategies to reduce the TCB and attack surface and maintain dedicated in-memory secure log environments.
% 

\vspace{0.2em}
\noindent
{\em \uppercase\expandafter{\romannumeral1}. Any component within the secure environment should not be shared with large existing system components.}
%
General-purpose layers (VMM and TZ used by~\cite{varun2023omnilog,shepherd2017emlog}) expose many interfaces to their clients (\eg feature-rich VMs), and hundreds of vulnerabilities have been found even in type-1 hypervisors and commercial TZ systems~\cite{chen2023security,cerdeira2020tzsok}.
%
As such, a secure environment for keeping logs should not rely on these layers to avoid sharing attack surfaces.
%
Otherwise, a simple vulnerability within a general client~\cite{chen2008overshadow,cerdeira2022rezone} can compromise the full system and the protected logs.
% 

% with large TCB and numerous interfaces~\cite{cerdeira2020tzsok,agache2020firecracker}.
% 
% If the secure environment shares components at the same privilege layers with them, it significantly increases the environment's attack surface and TCB.
% 


% Instead, \codename employs the privileged EL3 (SMM) for \sm alongside a {\em native but secured user-space} daemon for \hd (\cite{varun2023omnilog,shepherd2017emlog} use commodity trusted kernels).
% % 
% Unlike VMMs and TZ, EL3 is purposefully kept very small (\cref{sec:arm_background}), and provides a narrow interface (through \textcode{SMC}s) to the OS. 
% % 
% The \hd is designed to only accept remote input through a narrow memory-based communication channel that is secured end-to-end (using cryptographic protocols) with the administrator~(\cref{subsec:design_security_monitor}).
% % 
% Apart from that, the handling of the user-space daemon is securely delegated to the untrusted OS to keep its codebase small (please refer to the third strategy).
% % 

% {\em \uppercase\expandafter{\romannumeral1}. To reduce the attack surface, none of \codename's trusted components are shared with large existing system components (\eg VMM and TZ).}
% %
% Instead, \codename employs the privileged EL3 (SMM) for \sm alongside a {\em native but secured user-space} daemon for \hd (\cite{varun2023omnilog,shepherd2017emlog} use commodity trusted kernels).
% % 
% Unlike VMMs and TZ, EL3 is purposefully kept very small (\cref{sec:arm_background}), and provides a narrow interface (through \textcode{SMC}s) to the OS. 
% % 
% The \hd is designed to only accept remote input through a narrow memory-based communication channel that is secured end-to-end (using cryptographic protocols) with the administrator~(\cref{subsec:design_security_monitor}).
% % 
% Apart from that, the handling of the user-space daemon is securely delegated to the untrusted OS to keep its codebase small (please refer to the third strategy).
% % 

\vspace{0.2em}
\noindent
{\em \uppercase\expandafter{\romannumeral2}. The secure log environment should not reuse any large buggy codebase of commodity software.}
%
Besides a trusted kernel (tackled next), the largest buggy component of existing in-memory secure environments is their storage driver.
% 
This driver is required for log persistence and is typically adapted from commodity kernels like Linux (\eg over 10k LoC in a SATA driver), which has many bugs~\cite{guo2022driverlet,wang2022rttee}.
% 
To avoid transplanting bugs into the secure environment or increasing TCB, such codebases should not be leveraged.
% 

%
% Such a protected driver is required in the privileged \sm, ensuring log persistence.
% %
% Instead of porting a huge commodity driver into \sm, \sm employs a debloated driver synthesized through {\em driver record-and-replay}~\cite{guo2022driverlet,wang2022rttee}, by automatically recording a driver template through sample I/O tasks and replaying it inside \sm.
% %



% {\em \uppercase\expandafter{\romannumeral2}. To avoid reusing the large buggy codebase of commodity software within its trusted components, \codename leverages debloating.}
% %
% Besides a trusted kernel, the largest buggy component of an in-memory secure environment is its storage driver.
% %
% Such a protected driver is required in the privileged \sm, ensuring log persistence.
% %
% Instead of porting a huge commodity driver into \sm, \sm employs a debloated driver synthesized through {\em driver record-and-replay}~\cite{guo2022driverlet,wang2022rttee}, by automatically recording a driver template through sample I/O tasks and replaying it inside \sm.
% %
% While there are other choices, like porting and isolating a driver into \sm via memory-safe language, we choose the driver record-and-replay due to (a) easy-of-verification given such a debloated driver, and (b) easy-to-deploy as it can be automatically recorded (explained in \cref{subsec:design_offline}).
% %
% Nonetheless, the other approaches can be applied as well in the future.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\vspace{0.2em}
\noindent
{\em \uppercase\expandafter{\romannumeral3}. Log management tasks should be securely delegated to the OS without using a trusted kernel.}
%
Remote log management (\eg retrieval) is non-critical after OS compromise: administrators always recover the OS first.
%
Logs can be physically retrieved from the protected log storage during recovery.
%
Hence, we should not increase the secure log environment's TCB by using a trusted kernel for management tasks.
% 
Instead, these tasks should be delegated to the OS in a secure manner: if a log management request (\eg retrieval) succeeds, we should be able to verify that it was completed correctly.
% 

\adil{A reviewer complained that this section was too verbose.}

% The daemon (\hd) must be scheduled and requires networking services to communicate with remote administrators, but it cannot do so itself since it is in userspace.
% % 
% \codename does not emulate these services within \sm or deploy a trusted kernel~\cite{shepherd2017emlog,varun2023omnilog}, which increases its TCB considerably.
% %
% Instead, these services are delegated to the OS while interposed by \sm to ensure the integrity of \hd and network communication~(\cref{subsec:design_daemon}).
% % 
% % The daemon (\hd) process scheduling and system services (\eg network) are transparently supported by the native OS, while \sm 
% % protect it from the OS (\ie the untrusted OS is by no means allowed to access the daemon's memory space in any event).
% % %
% This aligns with the concept of {\em delegate-rather-than-emulate}~\cite{shinde2017panoply,hofmann2013inktag,hof2022blackbox,zhang2023shelter}, preventing expanding the TCB.
% %
% An organic byproduct of this approach is obviating the resource consumption associated with additional runtimes, such as the performance tax of a VM~\cite{ahmad2022hardlog} or OP-TEE kernel~\cite{optee-overhead}.
% %

% Although a compromised OS can kill the delegated \hd, deny the network services, pause the timer, or simply halt log capture, it cannot harm the integrity and availability of protected logs.
% %
% This is because (a) the secure environment and protected logs retain their integrity under the interposition of the \sm; (b) all protected logs will be persisted in secure storage, with their physical availability guaranteed by the \sm protected device driver; and (c) logs created post-OS compromise are deemed worthless~(\cref{subsec:threat_model})~\cite{ahmad2022hardlog,varun2023omnilog}, 
% negating the need for service support.\adil{Needs some work.}

% \begin{conclusionbox}
% {\bf Takeaway:}
% %
% {\em The secure environment should be kept small and avoid sharing attack surfaces with common components. 
% %
% Critical functions, including memory protection primitives for integrity and a protected storage driver for availability, should be kept debloated inside the environment.
% %
% Non-critical management functions (\ie the log daemon) should be securely delegated to the OS. 
% }
% \end{conclusionbox}
% \chuqi{TODO: use bullet points at the beginning of this section?}
%


==> tex/storage_protection.tex <==
\section{Storage Protection}
\label{sec:storage_protection}

To persist logs into protected storage, a block device driver exclusively for the secure monitor (SM) is necessary.
Moreover, providing such a driver without bloating the TCB is essential for \codename's principle (as stated in~\cref{subsec:system_principles}).

Porting a full-fledged driver from the OS to the SM is impractical due to its significant code size and TCB, leading to a larger attack surface~\cite{guo2022driverlet}.
For example, a SATA driver in Linux involves more than 10K lines of code with complex kernel dependencies and libraries.
Recent works~\cite{wang2022rttee,guo2022driverlet,park2023gpureplay} suggest to use \textit{record-and-replay} technique to synthesize a debloated driver template.
Typically, a block device can be viewed as a finite state machine (FSM).
Then, the driver can be templatized to a sequence of interactions for FSM state transitions which are I/O payload independent~\cite{guo2022driverlet}.
Thus, the goal is to record and model the device-driver interactions, rather than dealing with driver's complex codebase.
By doing so, SM can replay the recorded template interactions with dynamic values to accomplish I/O jobs.


\noindent\textbf{Driver template record.}
The recording phase is conducted before the system deployment.
A sample I/O job is then issued to the storage device. During this operation, the recorder tracks driver-device interactions:
(1) the sequence order and content of MMIO writes,
(2) the allocation of DMA memory and the I/O payload's location within this memory, and
(3) the storage device's triggered IRQ number along with the completion status set in the IRQ.
By generalizing the dynamic variables inside the recorded traces, \codename synthesizes a debloated driver template.

\noindent\textbf{Debloated driver initialization.}
During secure boot, SM initializes and protects the debloated driver interface in its memory space.
It reserves a DMA memory region and relies on the OS to map it to the storage device (i.e., \texttt{dma\_map\_sg}).
After mapping, SM configures \Aa{GPT}{NS} to restrict OS access to the DMA memory (\hwno{8}) and protects the driver's MMIO regions from the OS by editing \Aa{GPT}{NS}'s access permission (\hwno{7}).


The DMA memory is to hold I/O payloads (logs to persist). 
It is mapped into HD's address space during \textbf{C1} as the internal buffer for the manager thread (\circlewhite{3}).
In runtime, HD's manager thread requests the SM's primitive abstraction (\hwno{9}) to persist logs into storage.


\noindent\textbf{Poweroff management.}

==> tex/workflow.tex <==
\section{Workflow}
\label{sec:workflow}

At a high level, \codename leverages essential hardware primitives within a secure monitor to establish its protection pipeline, as illustrated in~\cref{fig:workflow}.

\adil{This workflow looks suspiciously like OmniLog. Think about if you could present it in a somewhat different way. Also too many headings}

\noindent\textbf{Secure monitor.}
\codename deploys a \textit{secure monitor} (SM) in the highest privilege level EL3 to abstract hardware primitives (shown in~\cref{tab:hw_abstraction}) required by system resource isolation.
During secure boot, SM initiates two GPTs: one for normal OS (\Aa{GPT}{NS}) and the other for the secure environment (\Aa{GPT}{HD}).
Thus, SM modulates memory access permissions, ensuring CPUs can only access dedicated memory view in their contexts.
\codename leverages a \textit{trampoline}~--~a segment of assembly code inside OS containing the secure monitor call (\texttt{smc})~--~to interact with SM and request the required primitive abstraction.
To ensure the legality of the invocation, a \textit{trusted gateway} inside the SM (\circleblack{A}) verifies the \texttt{smc} before executing the requested abstraction.

\noindent\textbf{Observability generation}. 
The in-kernel \textit{observability generator} records multi-level system events as logs to a \textit{current} kernel log buffer (\circleblack{1}--\circleblack{3\scriptsize{a}}) in an asynchronous and non-blocked manner.
After log generation, the control flow immediately resumes to the OS to continue its execution (\cref{subsec:obs_gen}).

\noindent\textbf{In-memory observability protection}.
To protect logs inside a kernel buffer, a \textit{flexible asynchronous protection scheme} $T_p$ is employed.
Specifically, a hardware timer periodically invokes the SM (\circleblack{3\scriptsize{b}}--\circleblack{A}) at an adjustable frequency of $T_p$ ($\le$~1 ms).
By configuring the buffer's permission to be inaccessible to the OS in \Aa{GPT}{NS} (\circlered{1}--\circlered{2\scriptsize{a}}), the SM swiftly secures the current log buffer from the OS.
Then, a new buffer is fetched from the \textit{buffer pool} (\circleblack{B}--\circleblack{3\scriptsize{c}}) for subsequent log generation (\cref{subsec:inmemory_obs_protection}).

\noindent\textbf{\codename Daemon (HD).} 
HD is a \textit{dedicated secure environment to log management} created and maintained by SM.
Its CPU execution context and memory space are isolated from the untrusted OS.
Once a buffer is secured from OS, the HD is scheduled to consume the buffer (\circlewhite{1}--\circlewhite{2}).
The HD leverages its preloaded exception vectors as a proxy (\circlewhite{A}--\circlewhite{B}) to interact with the SM (\circleblack{A}) to refill the buffer pool (\circlered{1}--\circlered{\Aa{2}{b}}) or further request OS services (\circleblack{B}--\circleblack{C}) such as network access.
Administrators can manage logs (\circlewhite{X}--\circlewhite{Z}) through a secure channel (e.g., TLS) to the HD (\cref{subsec:daemon_secure_environment}, \cref{subsec:daemon_realtime_execution}).

\noindent\textbf{Storage protection}.
To persist logs into protected storage, SM isolates a device driver template within its memory space to accomplish a debloated driver.
Only the HD's execution context or the SM can access the protected device (\circleblue{A}--\circleblue{B}) to issue log persistence commands.
SM also intercepts power events to ensure log persistence before system shutdown (\cref{subsec:design_storage_prot}).
